Precise determination of muon and EM shower contents from shower universality property

We present two new aspects of Extensive Air Shower (EAS) development universality allowing to make accurate estimation of muon and electromagnetic (EM) shower contents in two independent ways. In the first case, to get muon (or EM) signal in water Cherenkov detectors it is enough to know the vertical depth of shower maximum and the total signal. In the second case, the EM signal can be calculated from the primary particle energy and the zenith angle. In both cases the parameterizations of muon and EM signals are almost independent on primary particle nature, energy and zenith angle.

==> Makefile <==
# Copyright 2004 Chris Monson (monpublic@gmail.com)
# Latest version available at http://www.bouncingchairs.net/oss
#
#    This file is part of ``Chris Monson's Free Software''.
#
#    ``Chris Monson's Free Software'' is free software; you can redistribute it
#    and/or modify it under the terms of the GNU General Public License as
#    published by the Free Software Foundation, Version 2.
#
#    ``Chris Monson's Free Software'' is distributed in the hope that it will
#    be useful, but WITHOUT ANY WARRANTY; without even the implied warranty of
#    MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the GNU General
#    Public License for more details.
#
#    You should have received a copy of the GNU General Public License along
#    with ``Chris Monson's Free Software''; if not, write to the Free Software
#    Foundation, Inc., 59 Temple Place, Suite 330, Boston, MA  02111-1307  USA
#
#    It is also available on the web at http://www.gnu.org/copyleft/gpl.html
#
#    Note that using this makefile to build your documents does NOT place them
#    under the GPL unless you, the author, specifically do so.  In other words,
#    I, Chris Monson, the copyright holder and author of this makefile,
#    consider it impossible to ``link'' to this makefile in any way covered by
#    the GPL.
#
# TO OBTAIN INSTRUCTIONS FOR USING THIS FILE, RUN:
#    make help
#
fileinfo	:= LaTeX Makefile
author		:= Chris Monson
version		:= 2.1.23
svninfo		:= $$Id: Makefile 44 2008-10-23 16:30:20Z shiblon $$
#
# If you specify sources here, all other files with the same suffix
# will be treated as if they were _include_ files.
#onlysources.tex	:= main.tex
#onlysources.tex.sh	:=
#onlysources.rst	:=
#onlysources.fig	:=
#onlysources.gpi	:=
#onlysources.dot	:=
#onlysources.eps.gz	:=
#onlysources.eps	:=
#
# If you list files here, they will be treated as _include_ files
#includes.tex		:= file1.tex file2.tex
#includes.tex.sh	:=
#includes.rst		:=
#includes.fig		:=
#includes.gpi		:=
#includes.dot		:=
#includes.eps.gz	:=
#includes.eps		:=
#
# Alternatively (recommended), you can add those lines to a Makefile.ini file
# and it will get picked up automatically without your having to edit this
# Makefile.
-include Makefile.ini

# TODO:
# 	* Sometimes we get
# 		"mv: cannot stat '*.dvi.1st.make': No such file or directory"
# 		 on the second build (if nothing triggered a .d rebuild, but
# 		 the .dvi rule fired anyway).  To reproduce in the
# 		 dissertation directory:
#
#		 make clean
# 		 make byumsphd-example
# 		 make byumsphd-example
#
# KNOWN ISSUES:
#	* The following occurs:
#		file with: \usepackage{named}\bibliographystyle{named}
#		Compile
#		change to: \usepackage{apalike}\bibliographystyle{apalike}
#		Compile again -- BARF!
#
#		The workaround: make clean-nographics; make
#
#		Note that we may not be able to fix this.  LaTeX itself barfs
#		on this, not the makefile.  The very first invocation of LaTeX
#		(when something like this has happened) reads the existing .aux
#		file and discovers invalid commands like \citeauthoryear that
#		are only valid in the package that was just removed.  It then
#		tries to parse them and explodes.  It's not at all clear to me
#		how to fix this.  I tried removing the .aux files on the first
#		run of LaTeX, but that necessarily requires more subsequent
#		rebuilds on common edits.  There does not appear to be a
#		graceful solution to this issue.
#
# CHANGES:
# Chris Monson (2008-10-23):
# 	* Bumped version to 2.1.23
# 	* issue 23: fixed _check_programs to not use bash string subs
# Chris Monson (2008-09-02):
# 	* Bumped version to 2.1.22
# 	* Appled patch from Holger <yllohy@googlemail.com> to add include
# 		sources and some documentation updates.
# 	* Updated backup_patterns to be a bit more aggressive (also thanks to
# 		Holger)
# Chris Monson (2008-08-30):
# 	* Bumped version to 2.1.21
# 	* Added ability to specify onlysources.* variables to indicate the only
# 		files that should *not* be considered includes.  Thanks to Holger
# 		<yllohy@googlemail.com> for this patch.
# 	* Added an automatic include of Makefile.ini if it exists.  Allows
# 		settings to be made outside of this makefile.
# Chris Monson (2008-05-21):
# 	* Bumped version to 2.1.20
# 	* Added manual pstex compilation support (run make all-pstex first)
# 	* Removed all automatic pstex support.  It was totally breaking
# 		everything and is very hard to incorporate into the makefile
# 		concept because it requires LaTeX to *fail* before it can
# 		determine that it needs the files.
# Chris Monson (2008-04-17):
# 	* Bumped version to 2.1.19
# 	* Changed the pstex build hack to be on by default
# Chris Monson (2008-04-09):
# 	* Bumped version to 2.1.18
# 	* issue 16: fixed pstex build problems, seems nondeterministic.  Added
# 		gratuitious hack for testing: set PSTEX_BUILD_ALL_HACK=1.
# Chris Monson (2008-04-09):
# 	* Bumped version to 2.1.17
# 	* issue 20: fixed accumulation of <pid>*.make files - wildcard was
#		refusing to work on files that are very recently created.
# Chris Monson (2008-04-02):
# 	* Bumped version to 2.1.16
# 	* issue 19: Removed the use of "type" to fix broken "echo" settings
# Chris Monson (2008-03-27):
# 	* Bumped version to 2.1.15
# 	* issue 18: Favors binary echo over builtin, as binary understands -n
# 	* issue 16: Fixed handling of missing pstex_t files in the log
# 	* issue 9: Added .SECONDARY target for .pstex files
# Chris Monson (2008-03-21):
# 	* Bumped version to 2.1.14
# 	* Fixed broken aux file flattening, which caused included bibs to be
# 		missed.
# Chris Monson (2008-03-20):
# 	* Bumped version to 2.1.13
# 	* Changed error output colorization to show errors for missing files
# 		that are not graphics files.
# Chris Monson (2008-03-20):
# 	* Bumped version to 2.1.12
# 	* Fixed a regression introduced in r28 that makes bibtex fail when
# 		there is no index file present
# Chris Monson (2008-03-03):
# 	* Bumped version to 2.1.11
# 	* Fixed issue 11 (handle index files, reported by abachn)
# 	* Cleaned up some comments and help text
# Chris Monson (2008-01-24):
# 	* Bumped version to 2.1.10
#	* Fixed to work when 'sh' is a POSIX shell like 'dash'
# Chris Monson (2007-12-12):
# 	* Bumped version to 2.1.9
# 	* Fixed documentation and dependency graph for pstex files
# Chris Monson (2007-12-12):
# 	* Bumped version to 2.1.8
# 	* Added basic pstex_t support for fig files (Issue 9 by favonia)
# 		I still suggest that psfrag be used instead.
# Chris Monson (2007-10-16):
# 	* Bumped version to 2.1.7
# 	* Removed todo item: allow other comment directives for rst conversion
# 	* Added ability to use global rst style file _rststyle_._include_.tex
# 	* Added help text to that effect
# Chris Monson (2007-05-20):
# 	* Bumped version to 2.1.6
# 	* Changed default paper size for rst files
# 	* Added todo item: fix paper size for rst files
# 	* Added todo item: allow other comment directives for rst conversion
# Chris Monson (2007-04-02):
# 	* Bumped version to 2.1.5
# 	* Addressed Issue 7, incorrect .gpi.d generation in subdirectories
# Chris Monson (2007-03-28):
# 	* Bumped version to 2.1.4
# 	* Fixed syntax error in dot output
# Chris Monson (2007-03-01):
# 	* Bumped version to 2.1.3
# 	* Added reST to the included documentation
# 	* Fixed graphics and script generation to be settable in the
# 		environment.
# Chris Monson (2007-02-23):
# 	* Bumped version to 2.1.2
# 	* Added the ability to generate .tex files from .rst files
# Chris Monson (2006-10-17):
# 	* Bumped version to 2.1.1
# 	* Fixed includes from subdirectories (sed-to-sed slash escape problem)
# Chris Monson (2006-10-05):
# 	* Bumped version to 2.1.0 (pretty serious new feature added)
# 	* New feature: bib files can now be anywhere on the BIBINPUTS path
# 	* New programs: kpsewhich (with tetex) and xargs (BSD)
# Chris Monson (2006-09-28):
# 	* Bumped version to 2.0.9
# 	* Added ability to parse more than one bibliography
# Chris Monson (2006-06-01):
# 	* Bumped version to 2.0.8
# 	* Added .vrb to the list of cleaned files
# Chris Monson (2006-04-26):
# 	* Bumped version to 2.0.7
# 	* Fixed so that clean-nographics does not remove .gpi.d files
# 	* Removed jpg -> eps hack (not working properly -- just pre-convert)
# 	* Fixed so that postscript grayscale can be done with BSD sed
# Chris Monson (2006-04-25):
# 	* Bumped version to 2.0.6
# 	* Fixed so that changed toc, lot, lof, or out causes a rebuild
# Chris Monson (2006-04-17):
# 	* Bumped version to 2.0.5
# 	* Added jpg -> eps conversion target
# Chris Monson (2006-04-12):
# 	* Bumped version to 2.0.4
# 	* Fixed BSD sed invocation to not use \| as a branch delimiter
# 	* Added a comment section on what is and is not allowed in BSD sed
# 	* Made paper size handling more robust while I was at it
# 	* Fixed postscript RGB grayscale to use a weighted average
# 	* Fixed postscript HSB grayscale to convert to RGB first
# 	* Fixed a problem with rebuilding .bbl files
# Chris Monson (2006-04-11):
# 	* Bumped version to 2.0.3
# 	* Fixed some BSD sed problems: can't use \n in substitutions
# Chris Monson (2006-04-10):
# 	* Bumped version to 2.0.2
# 	* Once again removed ability to create .tex files from scripts
# 	* \includeonly works again
# Chris Monson (2006-04-09):
# 	* Bumped version to 2.0.1
# 	* Fixed grayscale postscript handling to be more robust
# 	* Added ability to generate ._gray_. files from eps and eps.gz
# 	* Added ability to clean ._gray_.eps files created from .eps files
# Chris Monson (2006-04-07):
# 	* Bumped version to 2.0.0
# 	* Removed clunky ability to create included .tex files from scripts
# 	* Added note in the help about included tex scripting not working
# 	* Fixed the .eps generation to delete %.gpihead.make when finished
# 	* Abandoned designs to use shell variables to create sed scripts
# 	* Abandoned __default__.tex.sh idea: it causes recursion with %: .
# 	* Removed web page to-do.  All items are now complete.
# 	* Added better grayscale conversion for dot figures (direct ps fixup).
# 	* Include files can now be scripted (at the expense of \includeonly).
# 	* Updated dependency graph to contain better node names.
# Chris Monson (2006-04-06):
# 	* Bumped version to 2.0b3
# 	* Top level includes now fail if there is no rule to build them
# 	* A helpful message is printed when they do fail
# 	* Grayscale has been changed to be ._gray_, other phonies use _ now, too
# 	* Grayscale handling has been completed
# 	* Changed _include_stems target to _includes target.
# 	* Fixed _includes target to be useful by itself.
# 	* Removed the ability to specify clean and build targets at once
# 	* Verified that epsfig works fine with current code
# 	* Fixed included scripts so that they are added to the dep files
# 	* Fixed so that graphics includes don't happen if they aren't for gpi
# 	* Fixed dot output to allow grayscale.
# Chris Monson (2006-04-05):
#	* Bumped version to 2.0b2
#	* Removed automatic -gray output.  It needs fixing in a bad way.
#	* Revamped dependency creation completely.
#	* Fixed conditional inclusion to actually work (test.nobuild.d, test.d).
#	* Fixed clean target to remove log targets
#	* Added the 'monochrome' word for gray gpi output
#	* Added a _check_gpi_files target that checks for common problems
#	* Changed the _version target into the version target (no _)
#	* Added better handling of grayscale files.  Use the .gray.pdf target.
#	* Fixed testing for rebuilds
# Chris Monson (2006-04-04):
#	* Bumped version to 2.0b1
#	* Changed colorization of output
#	* Made .auxbbl and .auxtex .make files secondary targets
#	* Shortened and simplified the final latex invocation loop
#	* Added version-specific output ($$i vs. $$$$i) in latex loop
#	* Added a build message for the first .dvi run (Building .dvi (0))
#	* Removed some build messages that most people don't care about.
#	* Simplified procedure for user-set colors -- simple text specification
#	* Fixed diff output to...not output.
#	* Fixed rerun bug -- detect not only when preceded with LaTeX Warning
#	* Sped up gpi plotting
#	* Added error handling and colorized output for gpi failure
#	* Documented color changing stuff.
#	* Now sort the flattened aux file to avoid false recompilation needs
#	* Added clean-nographics target
#	* Don't remove self.dvi file if self.aux is missing in the log
#	* Clarified some code.  Did some very minor adjusting.
# Chris Monson (2006-04-03):
#	* Bumped version to 2.0a7
#	* Added .dvi and .ps files as secondary files.
#	* Fixed handling of multiple run detection when includeonly is in use.
#	* Added code to flatten .aux files.
#	* Added more files as .SECONDARY prerequisites to avoid recompilation.
#	* Fixed the inputs generation to be much simpler and to use pipes.
#	* Added the dependency graph directly into the makefile.
#	* Changed flatten-aux to remove \@writefile \relax \newlabel, etc.
#	* Undid pipe changes with sed usage (BSD sed doesn't know -f-).
#	* Added a _check_programs target that tells you what your system has.
#	* Fixed an error in colorization that made unnecessary errors appear
#	* Added view targets.
#	* Updated help text.
#	* Augmented cookies so that .aux can trigger .bbl and .dvi rebuilds
#	* Added more informative error handling for dvips and ps2pdf
# Chris Monson (2006-04-02):
#	* Bumped version to 2.0a6
#	* Added indirection to .bbl dependencies to avoid rebuilding .bbl files
#	* Streamlined the diff invocation to eliminate an existence test
#	* Removed special shell quote escape variables
#	* Moved includes to a more prominent location
#	* Fixed .inputs.make to not contain .aux files
#	* Fixed embedding to use a file instead of always grepping.
#	* Added *.make.temp to the list of cleanable files
#	* Fixed Ruby.  It should now be supported properly.
#	* Now differentiate between all, default, and buildable files.
#	* Fixed to bail out on serious errors.
#	* Revised the handling of includable files.  Still working on it.
# Chris Monson (2006-03-31):
#	* Bumped version to 2.0a5
#	* Fixed a bug with LaTeX error detection (there can be spaces)
#	* Added .bbl support, simplifying everything and making it more correct
#	* Refactored some tests that muddy the code
#	* Did a little cleanup of some shell loops that can safely be make loops
#	* Added support for graphviz .dot files
#	* Made _all_programs output easier to read
#	* Added the ruby support that has long been advertised
#	* Font embedding was screwed up for PostScript -- now implicit
#	* Changed the generation of -gray.gpi files to a single command
#	* Changed any make-generated file that is not included from .d to .make
# Chris Monson (2006-03-30):
#	* Bumped version to 2.0a4
#	* Fixed a bug with very long graphics file names
#	* Added a todo entry for epsfig support
#	* Fixed a bug paper size bug: sometimes more than one entry appears
#	* Fixed DVI build echoing to display the number instead of process ID
#	* DVI files are now removed on first invocation if ANY file is missing
#	* Added a simple grayscale approach: if a file ends with -gray.gpi, it
#		is created from the corresponding .gpi file with a special
#		comment ##GRAY in its header, which causes coloring to be
#		turned off.
#	* Fixed a bug in the handling of .tex.sh files.  For some reason I had
#		neglected to define file stems for scripted output.
#	* Removed a trailing ; from the %.graphics dependencies
#	* Added dvips embedding (I think it works, anyway)
# Chris Monson (2006-03-29):
#	* Bumped version to 2.0a3
#	* Fixed error in make 3.79 with MAKEFILE_LIST usage
#	* Added the presumed filename to the _version output
#	* Added a vim macro for converting sed scripts to make commands
#	* Added gpi dependency support (plotting external files and loading gpi)
#	* Allow .gpi files to be ignored if called .include.gpi or .nobuild.gpi
#	* Fixed sed invocations where \+ was used.  BSD sed uses \{1,\}.
# Chris Monson (2006-03-28):
#	* Bumped version to 2.0a2
#	* Added SHELL_DEBUG and VERBOSE options
#	* Changed the default shell back to /bin/sh (unset, in other words)
#	* Moved .PHONY declarations closer to their targets
#	* Moved help text into its own define block to obtain better formatting
#	* Removed need for double-entry when adding a new program invocation
#	* Moved .SECONDARY declaration closer to its relevant occurrence
#	* Commented things more heavily
#	* Added help text about setting terminal and output in gnuplot
#	* Created more fine-grained clean targets
#	* Added a %.graphics target that generates all of %'s graphics
#	* Killed backward-compatible graphics generation (e.g., eps.gpi=gpi.eps)
#	* For now, we're just GPL 2, not 3.  Maybe it will change later
#	* Made the version and svninfo into variables
# Chris Monson (2006-03-27):
#	* Bumped version to 2.0a1
#	* Huge, sweeping changes -- automatic dependencies

# IMPORTANT!
#
# When adding to the following list, do not introduce any blank lines.  The
# list is extracted for documentation using sed and is terminated by a blank
# line.
#
# EXTERNAL PROGRAMS:
# = ESSENTIAL PROGRAMS =
# == Basic Shell Utilities ==
CAT		:= cat
CP		:= cp -f
DIFF		:= diff
ECHO		:= echo
EGREP		:= egrep
ENV		:= env
MV		:= mv -f
SED		:= sed
SORT		:= sort
TOUCH		:= touch
UNIQ		:= uniq
WHICH		:= which
XARGS		:= xargs
# == LaTeX (tetex-provided) ==
BIBTEX		:= bibtex
DVIPS		:= dvips
LATEX		:= latex
MAKEINDEX	:= makeindex
KPSEWHICH	:= kpsewhich
PS2PDF_NORMAL	:= ps2pdf
PS2PDF_EMBED	:= ps2pdf13
# = OPTIONAL PROGRAMS =
# == Makefile Color Output ==
TPUT		:= tput
# == TeX Generation ==
RST2LATEX	?= rst2latex.py
# == EPS Generation ==
DOT		?= dot		# GraphViz
FIG2DEV		?= fig2dev	# XFig
GNUPLOT		?= gnuplot	# GNUplot
GUNZIP		?= gunzip	# GZipped EPS
# == Beamer Enlarged Output ==
PSNUP		?= psnup
# == Viewing Stuff ==
VIEW_POSTSCRIPT	?= gv
VIEW_PDF	?= xpdf
VIEW_GRAPHICS	?= display

# This ensures that even when echo is a shell builtin, we still use the binary
# (the builtin doesn't always understand -n)
FIXED_ECHO	:= $(if $(findstring -n,$(shell $(ECHO) -n)),$(shell which echo),$(ECHO))
ECHO		:= $(if $(FIXED_ECHO),$(FIXED_ECHO),$(ECHO))

# SH NOTES
#
# On some systems, /bin/sh, which is the default shell, is not linked to
# /bin/bash.  While bash is supposed to be sh-compatible when invoked as sh, it
# just isn't.  This section details some of the things you have to stay away
# from to remain sh-compatible.
#
#	* File pattern expansion does not work for {}
#	* [ "$x" = "$y" ] has to be [ x"$x" x"$y" ]
#	* &> for stderr redirection doesn't work, use 2>&1 instead
#
# BSD SED NOTES
#
# BSD SED is not very nice compared to GNU sed, but it is the most
# commonly-invoked sed on Macs (being based on BSD), so we have to cater to
# it or require people to install GNU sed.  It seems like the GNU
# requirement isn't too bad since this makefile is really a GNU makefile,
# but apparently GNU sed is much less common than GNU make in general, so
# I'm supporting it here.
#
# Sad experience has taught me the following about BSD sed:
#
# 	* \+ is not understood to mean \{1,\}
# 	* \| is meaningless (does not branch)
# 	* \n cannot be used as a substitution character
# 	* ? does not mean \{0,1\}, but is literal
# 	* a\ works, but only reliably for a single line if subsequent lines
# 		have forward slashes in them (as is the case in postscript)
#
# For more info (on the Mac) you can consult
#
# man -M /usr/share/man re_format
#
# And look for the word "Obsolete" near the bottom.

#
# EXTERNAL PROGRAM DOCUMENTATION SCRIPT
#

# $(call output-all-programs,[<output file>])
define output-all-programs
	[ -f '$(this_file)' ] && \
	$(SED) \
		-e '/^[[:space:]]*#[[:space:]]*EXTERNAL PROGRAMS:/,/^$$/!d' \
		-e '/EXTERNAL PROGRAMS/d' \
		-e '/^$$/d' \
		-e '/^[[:space:]]*#/i\ '\
		-e 's/^[[:space:]]*#[[:space:]][^=]*//' \
		$(this_file) $(if $1,> '$1',) || \
	$(ECHO) "Cannot determine the name of this makefile."
endef

# If they misspell gray, it should still work.
GRAY	?= $(call get-default,$(GREY),)

#
# Utility Functions and Definitions
#

# While not exactly a make function, this vim macro is useful.  It takes a
# verbatim sed script and converts each line to something suitable in a command
# context.  Just paste the script's contents into the editor, yank this into a
# register (starting at '0') and run the macro once for each line of the
# original script:
#
# 0i	-e :s/\$/$$/eg
:s/'/'"'"'/eg
^Ela'A' \:noh
j

# don't call this directly - it is here to avoid calling wildcard more than
# once in remove-files.
remove-files-helper	= $(if $1,$(RM) $1,:)

# $(call remove-files,file1 file2)
remove-files		= $(call remove-files-helper,$(wildcard $1))

# This removes files without checking whether they are there or not.  This
# sometimes has to be used when the file is created by a series of shell
# commands, but there ends up being a race condition: make doesn't know about
# the file generation as quickly as the system does, so $(wildcard ...) doesn't
# work right.  Blech.
# $(call remove-temporary-files,filenames)
remove-temporary-files	= $(if $1,$(RM) $1,:)

# Create an identifier from a file name
# $(call cleanse-filename,filename)
cleanse-filename	= $(subst .,_,$(subst /,__,$1))

# Escape dots
# $(call escape-dots,str)
escape-dots		= $(subst .,\\.,$1)

# Test that a file exists
# $(call test-exists,file)
test-exists		= [ -e '$1' ]

# Copy file1 to file2 only if file2 doesn't exist or they are different
# $(call copy-if-different,sfile,dfile)
copy-if-different	= $(call test-different,$1,$2) && $(CP) '$1' '$2'
copy-if-exists		= $(call test-exists,$1) && $(CP) '$1' '$2'
move-if-different	= $(call test-different,$1,$2) && $(MV) '$1' '$2'
replace-if-different-and-remove	= \
	$(call test-different,$1,$2) \
	&& $(MV) '$1' '$2' \
	|| $(call remove-files,'$1')

# Note that $(DIFF) returns success when the files are the SAME....
# $(call test-different,sfile,dfile)
test-different		= ! $(DIFF) -q '$1' '$2' >/dev/null 2>&1
test-exists-and-different	= \
	$(call test-exists,$2) && $(call test-different,$1,$2)

# Return value 1, or value 2 if value 1 is empty
# $(call get-default,<possibly empty arg>,<default value if empty>)
get-default	= $(if $1,$1,$2)

# Gives a reassuring message about the failure to find include files
# $(call include-message,<list of include files>)
define include-message
$(strip \
$(if $(filter-out $(wildcard $1),$1),\
	$(shell $(ECHO) \
	"$(C_INFO)NOTE: You may ignore warnings about the"\
	"following files:" >&2;\
	$(ECHO) >&2; \
	$(foreach s,$(filter-out $(wildcard $1),$1),$(ECHO) '     $s' >&2;)\
	$(ECHO) "$(C_RESET)" >&2)
))
endef
# Characters that are hard to specify in certain places
space		:= $(empty) $(empty)
colon		:= \:
comma		:= ,

# Useful shell definitions
sh_true		:= :
sh_false	:= ! :

# Clear out the standard interfering make suffixes
.SUFFIXES:

# Turn off forceful rm (RM is usually mapped to rm -f)
ifdef SAFE_RM
RM	:= rm
endif

# Turn command echoing back on with VERBOSE=1
ifndef VERBOSE
QUIET	:= @
endif

# Turn on shell debugging with SHELL_DEBUG=1
# (EVERYTHING is echoed, even $(shell ...) invocations)
ifdef SHELL_DEBUG
SHELL	+= -x
endif

# Get the name of this makefile (always right in 3.80, often right in 3.79)
# This is only really used for documentation, so it isn't too serious.
ifdef MAKEFILE_LIST
this_file	:= $(word $(words $(MAKEFILE_LIST)),$(MAKEFILE_LIST))
else
this_file	:= $(wildcard GNUmakefile makefile Makefile)
endif

# Terminal color definitions

ifdef NO_COLOR
tput		=
else
tput		= $(shell $(TPUT) $1)
endif

black	:= $(call tput,setaf 0)
red	:= $(call tput,setaf 1)
green	:= $(call tput,setaf 2)
yellow	:= $(call tput,setaf 3)
blue	:= $(call tput,setaf 4)
magenta	:= $(call tput,setaf 5)
cyan	:= $(call tput,setaf 6)
white	:= $(call tput,setaf 7)
bold	:= $(call tput,bold)
uline	:= $(call tput,smul)
reset	:= $(call tput,sgr0)

#
# User-settable definitions
#
LATEX_COLOR_WARNING	?= magenta
LATEX_COLOR_ERROR	?= red
LATEX_COLOR_INFO	?= green
LATEX_COLOR_UNDERFULL	?= magenta
LATEX_COLOR_OVERFULL	?= red bold
LATEX_COLOR_PAGES	?= bold
LATEX_COLOR_BUILD	?= blue
LATEX_COLOR_GRAPHIC	?= yellow
LATEX_COLOR_DEP		?= green
LATEX_COLOR_SUCCESS	?= green bold
LATEX_COLOR_FAILURE	?= red bold

# Gets the real color from a simple textual definition like those above
# $(call get-color,ALL_CAPS_COLOR_NAME)
# e.g., $(call get-color,WARNING)
get-color	= $(subst $(space),,$(foreach c,$(LATEX_COLOR_$1),$($c)))

#
# STANDARD COLORS
#
C_WARNING	:= $(call get-color,WARNING)
C_ERROR		:= $(call get-color,ERROR)
C_INFO		:= $(call get-color,INFO)
C_UNDERFULL	:= $(call get-color,UNDERFULL)
C_OVERFULL	:= $(call get-color,OVERFULL)
C_PAGES		:= $(call get-color,PAGES)
C_BUILD		:= $(call get-color,BUILD)
C_GRAPHIC	:= $(call get-color,GRAPHIC)
C_DEP		:= $(call get-color,DEP)
C_SUCCESS	:= $(call get-color,SUCCESS)
C_FAILURE	:= $(call get-color,FAILURE)
C_RESET		:= $(reset)

#
# PRE-BUILD TESTS
#

# Check that clean targets are not combined with other targets (weird things
# happen, and it's not easy to fix them)
hascleangoals	:= $(if $(sort $(filter clean clean-%,$(MAKECMDGOALS))),1)
hasbuildgoals	:= $(if $(sort $(filter-out clean clean-%,$(MAKECMDGOALS))),1)
ifneq "$(hasbuildgoals)" ""
ifneq "$(hascleangoals)" ""
$(error $(C_ERROR)Clean and build targets specified together$(C_RESET)))
endif
endif

#
# VARIABLE DECLARATIONS
#

# Names of sed scripts that morph gnuplot files -- only the first found is used
GNUPLOT_SED	:= global-gpi.sed gnuplot.sed
GNUPLOT_GLOBAL	:= global._include_.gpi gnuplot.global

# Files of interest
all_files.tex		:= $(wildcard *.tex)
all_files.tex.sh	:= $(wildcard *.tex.sh)
all_files.rst		:= $(wildcard *.rst)
all_files.fig		:= $(wildcard *.fig)
all_files.gpi		:= $(wildcard *.gpi)
all_files.dot		:= $(wildcard *.dot)
all_files.eps.gz	:= $(wildcard *.eps.gz)
all_files.eps		:= $(wildcard *.eps)

# Utility function for getting all .$1 files that are to be ignored
#  * files listed in $(includes.$1)
#  * files not listed in $(onlysources.$1) if it is defined
ignore_files = \
  $(includes.$1) \
  $(if $(onlysources.$1),$(filter-out $(onlysources.$1), $(all_files.$1)))

# Patterns to never be allowed as source targets
ignore_patterns	:= %._include_

# Patterns allowed as source targets but not included in 'all' builds
nodefault_patterns := %._nobuild_ $(ignore_patterns)

# Utility function for getting targets suitable building
# $(call filter-buildable,suffix)
filter-buildable	= \
	$(filter-out $(call ignore_files,$1) \
		$(addsuffix .$1,$(ignore_patterns)),$(all_files.$1))

# Utility function for getting targets suitable for 'all' builds
# $(call filter-default,suffix)
filter-default		= \
	$(filter-out $(call ignore_files,$1) \
		$(addsuffix .$1,$(nodefault_patterns)),$(all_files.$1))

# Top level sources that can be built even when they are not by default
files.tex	:= $(filter-out %._gray_.tex,$(call filter-buildable,tex))
files.tex.sh	:= $(call filter-buildable,tex.sh)
files.rst	:= $(call filter-buildable,rst)
files.gpi	:= $(call filter-buildable,gpi)
files.dot	:= $(call filter-buildable,dot)
files.fig	:= $(call filter-buildable,fig)
files.eps.gz	:= $(call filter-buildable,eps.gz)

# Make all pstex targets secondary.  The pstex_t target requires the pstex
# target, and nothing else really depends on it, so it often gets deleted.
# This avoids that by allowing *all* fig files to be pstex targets, which is
# perfectly valid and causes no problems even if they're going to become eps
# files in the end.
.SECONDARY:	$(patsubst %.fig,%.pstex,$(files.fig))
.SECONDARY:	$(patsubst %.fig,%._gray_.pstex,$(files.fig))

# Top level sources that are built by default targets
default_files.tex	:= $(filter-out %._gray_.tex,$(call filter-default,tex))
default_files.tex.sh	:= $(call filter-default,tex.sh)
default_files.rst	:= $(call filter-default,rst)
default_files.gpi	:= $(call filter-default,gpi)
default_files.dot	:= $(call filter-default,dot)
default_files.fig	:= $(call filter-default,fig)
default_files.eps.gz	:= $(call filter-default,eps.gz)

# Utility function for creating larger lists of files
# $(call concat-files,suffixes,[prefix])
concat-files	= $(foreach s,$1,$($(if $2,$2_,)files.$s))

# Useful file groupings
all_files_source	:= $(call concat-files,tex,all)
all_files_scripts	:= $(call concat-files,tex.sh rst,all)
all_files_graphics	:= $(call concat-files,fig gpi eps.gz dot,all)

default_files_source	:= $(call concat-files,tex,default)
default_files_scripts	:= $(call concat-files,tex.sh rst,default)
default_files_graphics	:= $(call concat-files,fig gpi eps.gz dot,default)

files_source	:= $(call concat-files,tex)
files_scripts	:= $(call concat-files,tex.sh rst)
files_graphics	:= $(call concat-files,fig gpi eps.gz dot)

# Utility function for obtaining stems
# $(call get-stems,suffix,[prefix])
get-stems	= $(sort $($(if $2,$2_,)files.$1:%.$1=%))

# List of all stems (including ._include_ and ._nobuild_ file stems)
all_stems.tex		:= $(call get-stems,tex,all)
all_stems.tex.sh	:= $(call get-stems,tex.sh,all)
all_stems.rst		:= $(call get-stems,rst,all)
all_stems.fig		:= $(call get-stems,fig,all)
all_stems.gpi		:= $(call get-stems,gpi,all)
all_stems.dot		:= $(call get-stems,dot,all)
all_stems.eps.gz	:= $(call get-stems,eps.gz,all)
all_stems.eps		:= $(call get-stems,eps,all)

# List of all default stems (all default PDF targets):
default_stems.tex		:= $(call get-stems,tex,default)
default_stems.tex.sh		:= $(call get-stems,tex.sh,default)
default_stems.rst		:= $(call get-stems,rst,default)
default_stems.fig		:= $(call get-stems,fig,default)
default_stems.gpi		:= $(call get-stems,gpi,default)
default_stems.dot		:= $(call get-stems,dot,default)
default_stems.eps.gz		:= $(call get-stems,eps.gz,default)

# List of all stems (all possible bare PDF targets created here):
stems.tex		:= $(call get-stems,tex)
stems.tex.sh		:= $(call get-stems,tex.sh)
stems.rst		:= $(call get-stems,rst)
stems.fig		:= $(call get-stems,fig)
stems.gpi		:= $(call get-stems,gpi)
stems.dot		:= $(call get-stems,dot)
stems.eps.gz		:= $(call get-stems,eps.gz)

# Utility function for creating larger lists of stems
# $(call concat-stems,suffixes,[prefix])
concat-stems	= $(sort $(foreach s,$1,$($(if $2,$2_,)stems.$s)))

all_stems_source	:= $(call concat-stems,tex,all)
all_stems_script	:= $(call concat-stems,tex.sh rst,all)
all_stems_graphic	:= $(call concat-stems,fig gpi eps.gz dot,all)
all_stems_gray_graphic	:= $(addsuffix ._gray_,\
	$(all_stems_graphic) $(all_stems.eps) \
	)
all_stems_gg		:= $(sort \
	$(all_stems_graphic) $(all_stems_gray_graphic))
all_stems_ss		:= $(sort $(all_stems_source) $(all_stems_script))
all_stems_gray		:= $(addsuffix ._gray_,$(all_stems_ss))
all_stems_sg		:= $(sort $(all_stems_script) $(all_stems_gray))
all_stems_ssg		:= $(sort $(all_stems_ss) $(all_stems_gray))

default_stems_source	:= $(call concat-stems,tex,default)
default_stems_script	:= $(call concat-stems,tex.sh rst,default)
default_stems_graphic	:= $(call concat-stems,fig gpi eps.gz dot,default)
default_stems_gray_graphic	:= $(addsuffix ._gray_,$(default_stems_graphic))
default_stems_gg	:= $(sort \
	$(default_stems_graphic) $(default_stems_gray_graphic))
default_stems_ss	:= $(sort \
	$(default_stems_source) $(default_stems_script))
default_stems_gray	:= $(addsuffix ._gray_,$(default_stems_ss))
default_stems_sg	:= $(sort $(default_stems_script) $(default_stems_gray))
default_stems_ssg	:= $(sort $(default_stems_ss) $(default_stems_gray))

stems_source		:= $(call concat-stems,tex)
stems_script		:= $(call concat-stems,tex.sh rst)
stems_graphic		:= $(call concat-stems,fig gpi eps.gz dot)
stems_gray_graphic	:= $(addsuffix ._gray_,\
	$(stems_graphic) $(all_stems.eps))
stems_gg		:= $(sort $(stems_graphic) $(stems_gray_graphic))
stems_ss		:= $(sort $(stems_source) $(stems_script))
stems_gray		:= $(addsuffix ._gray_,$(stems_ss))
stems_sg		:= $(sort $(stems_script) $(stems_gray))
stems_ssg		:= $(sort $(stems_ss) $(stems_gray))

# Calculate names that can generate the need for an include file.  We can't
# really do this with patterns because it's too easy to screw up, so we create
# an exhaustive list.
allowed_source_suffixes	:= \
	pdf \
	ps \
	dvi \
	ind \
	bbl \
	aux \
	aux.make \
	d \
	tex \
	auxbbl.make \
	_graphics \
	_show
allowed_source_patterns		:= $(addprefix %.,$(allowed_source_suffixes))

allowed_graphic_suffixes	:= \
	eps \
	gpihead.make \
	gpi.d
allowed_graphic_patterns	:= $(addprefix %.,$(allowed_graphic_suffixes))

# All targets allowed to build documents
allowed_source_targets	:= \
	$(foreach suff,$(allowed_source_suffixes),\
	$(addsuffix .$(suff),$(stems_ssg)))

# All targets allowed to build graphics
allowed_graphic_targets	:= \
	$(foreach suff,$(allowed_graphic_suffixes),\
	$(addsuffix .$(suff),$(stems_gg)))

# All targets that build multiple documents (like 'all')
allowed_batch_source_targets	:= \
	all \
	all-pdf \
	all-ps \
	all-dvi \
	all-bbl \
	all-ind \
	show

# All targets that build multiple graphics (independent of document)
allowed_batch_graphic_targets	:= \
	all-graphics \
	all-pstex \
	all-gray-pstex \
	show-graphics

# Now we figure out which stuff is available as a make target for THIS RUN.
real_goals	:= $(call get-default,$(filter-out _includes,$(MAKECMDGOALS)),\
			all)

specified_source_targets	:= $(strip \
	$(filter $(allowed_source_targets) $(stems_ssg),$(real_goals)) \
	)

specified_batch_source_targets	:= $(strip \
	$(filter $(allowed_batch_source_targets),$(real_goals)) \
	)

specified_graphic_targets	:= $(strip \
	$(filter $(allowed_graphic_targets),$(real_goals)) \
	)

specified_batch_graphic_targets	:= $(strip \
	$(filter $(allowed_batch_graphic_targets),$(real_goals)) \
	)

specified_gpi_targets	:= $(patsubst %.gpi,%.eps,\
	$(filter $(patsubst %.eps,%.gpi,$(specified_graphic_targets)),\
		$(all_files.gpi)) \
	)

# Determine which .d files need including from the information gained above.
# This is done by first checking whether a batch target exists.  If it does,
# then all *default* stems are used to create possible includes (nobuild need
# not apply for batch status).  If no batch targets exist, then the individual
# targets are considered and appropriate includes are taken from them.
source_stems_to_include	:= \
	$(sort\
	$(if $(specified_batch_source_targets),\
		$(default_stems_ss),\
		$(foreach t,$(specified_source_targets),\
		$(foreach p,$(allowed_source_patterns),\
			$(patsubst $p,%,$(filter $p $(stems_ssg),$t)) \
		)) \
	))

# Determine which .gpi.d files are needed using the above information.  We
# first check whether a batch target is specified, then check individual
# graphics that may have been specified.
graphic_stems_to_include	:= \
	$(sort\
	$(if $(specified_batch_graphic_targets),\
		$(default_stems.gpi),\
		$(foreach t,$(specified_gpi_targets),\
		$(foreach p,$(allowed_graphic_patterns),\
			$(patsubst $p,%,$(filter $p,$t)) \
		)) \
	))

# All dependencies for the 'all' targets
all_pdf_targets		:= $(addsuffix .pdf,$(stems_ssg))
all_ps_targets		:= $(addsuffix .ps,$(stems_ssg))
all_dvi_targets		:= $(addsuffix .dvi,$(stems_ssg))
all_tex_targets		:= $(addsuffix .tex,$(stems_sg))
all_d_targets		:= $(addsuffix .d,$(stems_ssg))
all_graphics_targets	:= $(addsuffix .eps,$(stems_gg))
all_pstex_targets	:= $(addsuffix .pstex_t,$(stems.fig))
all_gray_pstex_targets	:= $(addsuffix ._gray_.pstex_t,$(stems.fig))

all_known_graphics	:= $(sort $(all_graphics_targets) $(wildcard *.eps))

default_pdf_targets	:= $(addsuffix .pdf,$(default_stems_ss))
default_ps_targets	:= $(addsuffix .ps,$(default_stems_ss))
default_dvi_targets	:= $(addsuffix .dvi,$(default_stems_ss))

# Extensions generated by LaTeX invocation that can be removed when complete
rm_ext		:= \
	log aux dvi ps pdf blg bbl out nav snm toc lof lot pfg fls vrb \
	idx ind ilg lox
backup_patterns	:= *~ *.bak *.backup

graph_stem	:= _graph

# All LaTeX-generated files that can be safely removed

rm_tex := \
	$(foreach e,$(rm_ext),$(addsuffix .$e,$(all_stems_source))) \
	$(foreach e,$(rm_ext) tex,$(addsuffix .$e,$(all_stems_sg))) \
	$(addsuffix .log,$(all_ps_targets) $(all_pdf_targets)) \
	$(addsuffix .*.log,$(stems_graphic))

# These are the files that will affect .gpi transformation for all .gpi files.
#
# Use only the first one found.  Backward compatible values are at the end.
# Note that we use foreach, even though wildcard also returns a list, to ensure
# that the order in the uppercase variables is preserved.  Directory listings
# provide no such guarantee, so we avoid relying on them.
gpi_sed		:= $(strip \
	$(firstword $(foreach f,$(GNUPLOT_SED),$(wildcard $f))))
gpi_global	:= $(strip \
	$(firstword $(foreach f,$(GNUPLOT_GLOBAL),$(wildcard $f))))

#
# Functions used in generating output
#

# Outputs all source dependencies to stdout.  The first argument is the file to
# be parsed, the second is a list of files that will show up as dependencies in
# the new .d file created here.
#
# NOTE: BSD sed does not understand \|, so we have to do something more
# clunky to extract suitable extensions.
#
# $(call get-inputs,<parsed file>,<target files>)
define get-inputs
$(SED) \
-e '/^INPUT/!d' \
-e 's!^INPUT \(\./\)\{0,1\}!$2: !' \
-e '/\.tex$$/p' \
-e '/\.cls$$/p' \
-e '/\.sty$$/p' \
-e 'd' \
$1 | $(SORT) | $(UNIQ)
endef

# Outputs all of the graphical dependencies to stdout.  The first argument is
# the stem of the source file being built, the second is a list of suffixes
# that will show up as dependencies in the generated .d file.
#
# $(call get-graphics,<parsed file>,<target files>)
define get-graphics
$(SED) \
-e '/^File:/!d' \
-e 'N' \
-e 's/\n//g' \
-e '/Graphic file/!d' \
-e 's/^File: //' \
-e 's/ Graphic.*$$//' \
-e '/^\(.*\)\(\.[^.]*\)$$/{' \
-e   's//$2: \1\2/' \
-e   'p' \
-e   's/[^:]*: \(.*\)\(\.[^.]*\)$$/-include \1.gpi.d/' \
-e   'p' \
-e   'd' \
-e '}' \
$1 | $(SORT) | $(UNIQ)
endef

# Checks for build failure due to pstex inclusion, and gives instructions.
#
# $(call die-on-pstexs,<parsed file>)
define die-on-pstexs
if $(EGREP) -q '^! LaTeX Error: File .*\.pstex.* not found' $1; then \
	$(ECHO) "$(C_ERROR)Missing pstex_t file(s)$(C_RESET)"; \
	$(ECHO) "$(C_ERROR)Please run$(C_RESET)"; \
	$(ECHO) "$(C_ERROR)  make all-pstex$(C_RESET)"; \
	$(ECHO) "$(C_ERROR)before proceeding.$(C_RESET)"; \
	exit 1; \
fi
endef

# Outputs all index files to stdout.  Arg 1 is the source stem, arg 2 is the
# list of targets for the discovered dependency.
#
# $(call get-inds,<parsed file>,<target files>)
define get-inds
$(SED) \
-e 's/^No file \(.*\)\.ind\.$$/$2: \1.ind/p' \
-e 'd' \
$1 | $(SORT) | $(UNIQ)
endef


# Outputs all bibliography files to stdout.  Arg 1 is the source stem, arg 2 is
# a list of targets for each dependency found.
#
# The script kills all lines that do not contain bibdata.  Remaining lines have
# the \bibdata macro and delimiters removed to create a dependency list.  A
# trailing comma is added, then all adjacent commas are collapsed into a single
# comma.  Then commas are replaced with the string .bib[space], and the
# trailing space is killed off.  This produces a list of space-delimited .bib
# filenames, which is what the make dep file expects to see.
#
# $(call get-bibs,<aux file>,<targets>)
define get-bibs
$(SED) \
-e '/^\\bibdata/!d' \
-e 's/\\bibdata{\([^}]*\)}/\1,/' \
-e 's/,\{2,\}/,/g' \
-e 's/,/.bib /g' \
-e 's/ \{1,\}$$//' \
$1 | $(XARGS) $(KPSEWHICH) - | \
$(SED) \
-e 's/^/$2: /' | \
\$(SORT) | $(UNIQ)
endef

# Makes a an aux file that only has stuff relevant to the dvi in it
# $(call make-auxdvi-file,<flattened-aux>,<new-aux>)
define make-auxdvi-file
$(SED) \
-e '/^\\newlabel/!d' \
$1 > $2
endef

# Makes an aux file that only has stuff relevant to the bbl in it
# $(call make-auxbbl-file,<flattened-aux>,<new-aux>)
define make-auxbbl-file
$(SED) \
-e '/^\\newlabel/d' \
$1 > $2
endef

# Makes a .gpi.d file from a .gpi file
# $(call make-gpi-d,<.gpi>,<.gpi.d>)
define make-gpi-d
$(ECHO) '# vim: ft=make' > $2; \
$(ECHO) 'ifndef INCLUDED_$(call cleanse-filename,$2)' >> $2; \
$(ECHO) 'INCLUDED_$(call cleanse-filename,$2) = 1' >> $2; \
$(call get-gpi-deps,$1,$(addprefix $(2:%.gpi.d=%).,eps gpi.d)) >> $2; \
$(ECHO) 'endif' >> $2;
endef

# Parse .gpi files for data and loaded dependencies, output to stdout
#
# The sed script here tries to be clever about obtaining valid
# filenames from the gpi file.  It assumes that the plot command starts its own
# line, which is not too difficult a constraint to satisfy.
#
# This command script also generates 'include' directives for every 'load'
# command in the .gpi file.  The load command must appear on a line by itself
# and the file it loads must have the suffix .gpi.  If you don't want it to be
# compiled when running make graphics, then give it a suffix of ._include_.gpi.
#
# $(call get-gpi-deps,<gpi file>,<targets>)
define get-gpi-deps
$(SED) \
-e '/^[[:space:]]*s\{0,1\}plot/,/[^\\]$$/{' \
-e ' H' \
-e ' /[^\\]$$/{' \
-e '  s/.*//' \
-e '  x' \
-e '  s/\\\{0,1\}\n//g' \
-e '  s/^[[:space:]]*s\{0,1\}plot[[:space:]]*\(\[[^]]*\][[:space:]]*\)*/,/' \
-e '  s/[[:space:]]*\(['\''"][^'\''"]*['\''"]\)\{0,1\}[^,]*/\1/g' \
-e '  s/,['\''"]-\{0,1\}['\''"]//g' \
-e '  s/[,'\''"]\{1,\}/ /g' \
-e '  s!.*!$2: &!' \
-e '  p' \
-e ' }' \
-e ' d' \
-e '}' \
-e 's/^[[:space:]]*load[[:space:]]*['\''"]\([^'\''"]*\.gpi\)['\''"].*$$/-include \1.d/p' \
-e 'd' \
$1
endef

# Colorizes real, honest-to-goodness LaTeX errors that can't be overcome with
# recompilation.
#
# Note that we only ignore file not found errors for things that we know how to
# build, like graphics files.
#
# $(call colorize-latex-errors,<log file>)
define colorize-latex-errors
$(SED) \
-e '/^! LaTeX Error: File .*eps'"'"' not found\.$$/d' \
-e '/^! LaTeX Error: Cannot determine size/d' \
-e '/^! /,/^$$/{' \
-e '  H' \
-e '  /^$$/{' \
-e '    x' \
-e '    s/^.*$$/$(C_ERROR)&$(C_RESET)/' \
-e '    p' \
-e '  }' \
-e '}' \
-e 'd' \
$1
endef

# Colorize Makeindex errors
define colorize-makeindex-errors
$(SED) \
-e '/^!! /{' \
-e '  N' \
-e '  s/^.*$$/$(C_ERROR)&$(C_RESET)/' \
-e '  p' \
-e '}' \
-e 'd' \
$1
endef

# Colorize GNUplot errors
#
# $(call colorize-gnuplot-errors,<log file>)
define colorize-gnuplot-errors
$(SED) \
-e '/^gnuplot>/,/^$$/{' \
-e '  s/^gnuplot.*/$(C_ERROR)&/' \
-e '  s/^$$/$(C_RESET)/' \
-e '  p' \
-e '}' \
-e 'd' \
$1
endef

# Colorize GraphViz errors
#
# $(call colorize-dot-errors,<log file>)
define colorize-dot-errors
$(SED) \
-e '/^Error:/,/context:/s/.*/$(C_ERROR)&$(C_RESET)/p' \
-e 's/^Warning:.*/$(C_WARNING)&$(C_RESET)/p' \
-e 'd' \
$1
endef

# Get all important .aux files from the top-level .aux file and merges them all
# into a single file, which it outputs to stdout.
#
# $(call flatten-aux,<toplevel aux>,<output file>)
define flatten-aux
$(SED) \
-e '/\\@input{\(.*\)}/{' \
-e     's//\1/' \
-e     's![.:]!\\&!g' \
-e     'h' \
-e     's!.*!\\:\\\\@input{&}:{!' \
-e     'p' \
-e     'x' \
-e     's/\\././g' \
-e     's/.*/r &/p' \
-e     's/.*/d/p' \
-e     's/.*/}/p' \
-e     'd' \
-e '}' \
-e 'd' \
'$1' > "$1.$$$$.sed.make"; \
$(SED) -f "$1.$$$$.sed.make" '$1' > "$1.$$$$.make"; \
$(SED) \
-e '/^\\relax/d' \
-e '/^\\bibcite/d' \
-e 's/^\(\\newlabel{[^}]\{1,\}}\).*/\1/' \
"$1.$$$$.make" | $(SORT) > '$2'; \
$(call remove-temporary-files,$1.$$$$.make $1.$$$$.sed.make)
endef

# Generate pdf from postscript
ps2pdf_normal	:= $(PS2PDF_NORMAL)
ps2pdf_embedded	:= \
	$(PS2PDF_EMBED) \
	-dPDFSETTINGS=/printer \
	-dEmbedAllFonts=true \
	-dSubsetFonts=true \
	-dMaxSubsetPct=100

# Colorize LaTeX output.
color_tex	:= \
	$(SED) \
	-e '/^[[:space:]]*Output written/{' \
	-e ' s/.*(\([^)]\{1,\}\)).*/Success!  Wrote \1/' \
	-e ' s/[[:digit:]]\{1,\}/$(C_PAGES)&$(C_RESET)/g' \
	-e ' s/Success!/$(C_SUCCESS)&$(C_RESET)/g' \
	-e '}' \
	-e 's/^! *LaTeX Error:.*/$(C_ERROR)&$(C_RESET)/' -e 't' \
	-e 's/^LaTeX Warning:.*/$(C_WARNING)&$(C_RESET)/' -e 't' \
	-e 's/^Underfull.*/$(C_UNDERFULL)&$(C_RESET)/' -e 't' \
	-e 's/^Overfull.*/$(C_OVERFULL)&$(C_RESET)/' -e 't' \
	$(if $(VERBOSE),,-e 'd')

# Colorize BibTeX output.
color_bib	:= \
	$(SED) \
	-e 's/^Warning--.*/$(C_WARNING)&$(C_RESET)/' -e 't' \
	-e '/---/,/^.[^:]/{' \
	-e '  H' \
	-e '  /^.[^:]/{' \
	-e '    x' \
	-e '    s/\n\(.*\)/$(C_ERROR)\1$(C_RESET)/' \
	-e '	p' \
	-e '    s/.*//' \
	-e '    h' \
	-e '    d' \
	-e '  }' \
	-e '  d' \
	-e '}' \
	-e '/(.*error.*)/s//$(C_ERROR)&$(C_RESET)/' \
	$(if $(VERBOSE),,-e 'd')


# Make beamer output big enough to print on a full page.  Landscape doesn't
# seem to work correctly.
enlarge_beamer	= $(PSNUP) -l -1 -W128mm -H96mm -pletter

# $(call test-run-again,<source stem>)
test-run-again	= $(EGREP) -q '^(.*Rerun .*|No file $1\.[^.]+\.)$$' $1.log

# This tests whether the dvi target should be run at all, from viewing the log
# file.
# $(call test-log-for-need-to-run,<source stem>)
define test-log-for-need-to-run
$(SED) \
-e '/^No file $(call escape-dots,$1)\.aux\./d' \
$1.log \
| $(EGREP) -q '^(.*Rerun .*|No file $1\.[^.]+\.|LaTeX Warning: File.*)$$'
endef

# LaTeX invocations
#
# $(call latex,<tex file>,[<extra LaTeX args>])
run-latex	= $(LATEX) --interaction=batchmode $(if $2,$2,) $1 > /dev/null

# $(call latex-color-log,<LaTeX stem>)
latex-color-log	= $(color_tex) $1.log

# $(call run-makeindex,<tex stem>)
define run-makeindex
success=1; \
if ! $(MAKEINDEX) -q $1.idx > /dev/null || $(EGREP) -q '^!!' $1.ilg; then \
	$(call colorize-makeindex-errors,$1.ilg); \
	success=0; \
fi; \
[ "$$success" = "1" ] && $(sh_true) || $(sh_false);
endef

# BibTeX invocations
#
# $(call run-bibtex,<tex stem>)
run-bibtex	= $(BIBTEX) $1 | $(color_bib)


# $(call convert-gpi,<gpi file>,<eps file>,[gray])
define convert-gpi
$(ECHO) 'set terminal postscript enhanced eps' \
$(call get-default,$(strip \
$(firstword \
	$(shell \
		$(SED) \
			-e 's/^\#\#FONTSIZE=\([[:digit:]]\{1,\}\)/\1/p' \
			-e 'd' \
			$1 $(strip $(gpi_global)) \
	) \
) \
),22) \
$(strip $(if $3,monochrome,$(if \
$(shell $(EGREP) '^\#\#[[:space:]]*GRAY[[:space:]]*$$' $< $(gpi_global)),\
,color))) > $1head.make; \
$(ECHO) 'set output "$2"' >> $1head.make; \
$(if $(gpi_global),$(CAT) $(gpi_global) >> $1head.make;,) \
fnames='$1head.make $1';\
$(if $(gpi_sed),\
	$(SED) -f '$(gpi_sed)' $$fnames > $1.temp.make; \
	fnames=$1.temp.make;,\
) \
success=1; \
if ! $(GNUPLOT) $$fnames 2>$1.log; then \
	$(call colorize-gnuplot-errors,$1.log); \
	success=0; \
fi; \
$(if $(gpi_sed),$(call remove-temporary-files,$1.temp.make);,) \
$(call remove-temporary-files,$1head.make); \
[ "$$success" = "1" ] && $(sh_true) || $(sh_false);
endef

# Creation of .eps files from .fig files
# $(call convert-fig,<fig file>,<eps file>,[gray])
convert-fig	= $(FIG2DEV) -L eps $(if $3,-N,) $1 $2

# Creation of .pstex files from .fig files
# $(call convert-fig-pstex,<fig file>,<pstex file>)
convert-fig-pstex	= $(FIG2DEV) -L pstex $1 $2 > /dev/null 2>&1

# Creation of .pstex_t files from .fig files
# $(call convert-fig-pstex-t,<fig file>,<pstex file>,<pstex_t file>)
convert-fig-pstex-t	= $(FIG2DEV) -L pstex_t -p $3 $1 $2 > /dev/null 2>&1

# Creation of .tex files from .rst files
# TODO: Fix paper size so that it can be specified in the file itself
# $(call convert-rst,<rst file>,<tex file>)
rst_style_file=$(wildcard _rststyle_._include_.tex)
define convert-rst
$(RST2LATEX) \
	--documentoptions=letterpaper \
	$(if $(rst_style_file),--stylesheet=$(rst_style_file),) \
	$1 $2
endef

# Converts .eps.gz files into .eps files
#
# $(call convert-epsgz,<eps.gz file>,<eps file>,[gray])
convert-epsgz	= $(GUNZIP) -c '$1' $(if $3,| $(call kill-ps-color)) > '$2'

# Converts .eps files into .eps files (usually a no-op, but can make grayscale)
#
# $(call convert-eps,<in file>,<out file>,[gray])
convert-eps	= $(if $3,$(call kill-ps-color) $1 > $2)

# The name of the file containing special postscript commands for grayscale
gray_eps_file	:= gray.eps.make

# Changes sethsbcolor and setrgbcolor calls in postscript to always produce
# grayscale.  In general, this is accomplished by writing new versions of those
# functions into the user dictionary space, which is looked up before the
# global or system dictionaries (userdict is one of the permanent dictionaries
# in postscript and is not read-only like systemdict).
#
# For setrgbcolor, the weighted average of the triple is computed and the
# triple is replaced with three copies of that average before the original
# procedure is called: .299R + .587G + .114B
#
# For sethsbcolor, the color is first converted to RGB, then to grayscale by
# the new setrgbcolor operator as described above.  Why is this done?
# Because simply using the value component will tend to make pure colors
# white, a very undesirable thing.  Pure blue should not translate to white,
# but to some level of gray.  Conversion to RGB does the right thing.  It's
# messy, but it works.
#
# From
# http://en.wikipedia.org/wiki/HSV_color_space#Transformation_from_HSV_to_RGB,
# HSB = HSV (Value = Brightness), and the formula used to convert to RGB is
# as follows:
#
# Hi = int(floor(6 * H)) mod 6
# f = 6 * H - Hi
# p = V(1-S)
# q = V(1-fS)
# t = V(1-(1-f)S)
# if Hi = 0: R G B <-- V t p
# if Hi = 1: R G B <-- q V p
# if Hi = 2: R G B <-- p V t
# if Hi = 3: R G B <-- p q V
# if Hi = 4: R G B <-- t p V
# if Hi = 5: R G B <-- V p q
#
# The messy stack-based implementation is below
# $(call create-gray-eps-file,filename)
define create-gray-eps-file
$(ECHO) -n -e '\
/OLDRGB /setrgbcolor load def\n\
/setrgbcolor {\n\
    .114 mul exch\n\
    .587 mul add exch\n\
    .299 mul add\n\
    dup dup\n\
    OLDRGB\n\
} bind def\n\
/OLDHSB /sethsbcolor load def\n\
/sethsbcolor {\n\
    2 index                     % H V S H\n\
    6 mul floor cvi 6 mod       % Hi V S H\n\
    3 index                     % H Hi V S H\n\
    6 mul                       % 6H Hi V S H\n\
    1 index                     % Hi 6H Hi V S H\n\
    sub                         % f Hi V S H\n\
    2 index 1                   % 1 V f Hi V S H\n\
    4 index                     % S 1 V f Hi V S H\n\
    sub mul                     % p f Hi V S H\n\
    3 index 1                   % 1 V p f Hi V S H\n\
    6 index                     % S 1 V p f Hi V S H\n\
    4 index                     % f S 1 V p f Hi V S H\n\
    mul sub mul                 % q p f Hi V S H\n\
    4 index 1 1                 % 1 1 V q p f Hi V S H\n\
    5 index                     % f 1 1 V q p f Hi V S H\n\
    sub                         % (1-f) 1 V q p f Hi V S H\n\
    8 index                     % S (1-f) 1 V q p f Hi V S H\n\
    mul sub mul                 % t q p f Hi V S H\n\
    4 -1 roll pop               % t q p Hi V S H\n\
    7 -2 roll pop pop           % t q p Hi V\n\
    5 -2 roll                   % Hi V t q p\n\
    dup 0 eq\n\
    {1 index 3 index 6 index}\n\
    {\n\
        dup 1 eq\n\
        {3 index 2 index 6 index}\n\
        {\n\
            dup 2 eq\n\
            {4 index 2 index 4 index}\n\
            {\n\
                dup 3 eq\n\
                {4 index 4 index 3 index}\n\
                {\n\
                    dup 4 eq\n\
                    {2 index 5 index 3 index}\n\
                    {\n\
                        dup 5 eq\n\
                        {1 index 5 index 5 index}\n\
                        {0 0 0}\n\
                        ifelse\n\
                    }\n\
                    ifelse\n\
                }\n\
                ifelse\n\
            }\n\
            ifelse\n\
        }\n\
        ifelse\n\
    }\n\
    ifelse                      % B G R Hi V t q p\n\
    setrgbcolor\n\
    5 {pop} repeat\n\
} bind def\n'\
> $1
endef

# This actually inserts the color-killing code into a postscript file
# $(call kill-ps-color)
define kill-ps-color
$(SED) -e '/%%EndComments/r $(gray_eps_file)'
endef

# Converts graphviz .dot files into .eps files
# Grayscale is not directly supported by dot, so we pipe it through fig2dev in
# that case.
# $(call convert-dot,<dot file>,<eps file>,<log file>,[gray])
define convert-dot
$(DOT) -Tps '$1' 2>'$3' $(if $4,| $(call kill-ps-color)) > '$2'; \
$(call colorize-dot-errors,$3)
endef

# Convert DVI to Postscript
# $(call make-ps,<dvi file>,<ps file>,<log file>,[<paper size>])
make-ps		= \
	$(DVIPS) -R0 -o '$2' $(if $(filter-out BEAMER,$4),-t$(firstword $4),) '$1' \
		$(if $(filter BEAMER,$4),| $(enlarge_beamer)) > $3 2>&1

# Convert Postscript to PDF
# $(call make-pdf,<ps file>,<pdf file>,<log file>,<embed file>)
make-pdf	= \
	$(if $(filter 1,$(shell $(CAT) '$4')),\
		$(ps2pdf_embedded),\
		$(ps2pdf_normal)) '$1' '$2' > $3 2>&1

# Display information about what is being done
# $(call echo-build,<output file>,[<run number>])
echo-build	= $(ECHO) "$(C_BUILD)= $1 --> $2$(if $3, ($3),) =$(C_RESET)"
echo-graphic	= $(ECHO) "$(C_GRAPHIC)= $1 --> $2 =$(C_RESET)"
echo-dep	= $(ECHO) "$(C_DEP)= $1 --> $2 =$(C_RESET)"

# Display a list of something
# $(call echo-list,<values>)
echo-list	= for x in $1; do $(ECHO) "$$x"; done

#
# DEFAULT TARGET
#

.PHONY: all
all: $(default_pdf_targets) ;

.PHONY: all-pdf
all-pdf: $(default_pdf_targets) ;

.PHONY: all-ps
all-ps: $(default_ps_targets) ;

.PHONY: all-dvi
all-dvi: $(default_dvi_targets) ;

#
# VIEWING TARGET
#
.PHONY: show
show: all
	$(QUIET)for x in $(default_pdf_targets); do \
		[ -e "$$x" ] && $(VIEW_PDF) $$x & \
	done

#
# INCLUDES
#
source_includes	:= $(addsuffix .d,$(source_stems_to_include))
graphic_includes := $(addsuffix .gpi.d,$(graphic_stems_to_include))

# Include only the dependencies used
ifneq "" "$(source_includes)"
include $(source_includes)$(call include-message,$(source_includes))
endif
ifneq "" "$(graphic_includes)"
include $(graphic_includes)$(call include-message,$(graphic_includes))
endif

#
# MAIN TARGETS
#

%: %.pdf ;

# This builds and displays the wanted file.
.PHONY: $(addsuffix ._show,$(stems_ssg))
%._show: %.pdf
	$(QUIET)$(VIEW_PDF) $< &

.SECONDARY: $(all_pdf_targets)
%.pdf: %.ps %.embed.make
	$(QUIET)$(call echo-build,$<,$@)
	$(QUIET)$(call make-pdf,$<,$@.temp,$@.log,$*.embed.make); \
	if [ x"$$?" = x"0" ]; then \
	    $(if $(VERBOSE),$(CAT) $@.log,:); \
	    $(MV) '$@.temp' '$@'; \
	else \
	    $(CAT) $@.log; \
	    $(call remove-temporary-files,'$@.temp'); \
	    $(sh_false); \
	fi

.SECONDARY: $(all_ps_targets)
%.ps: %.dvi %.paper.make
	$(QUIET)$(call echo-build,$<,$@)
	$(QUIET)$(call make-ps,$<,$@.temp,$@.log,\
			$(firstword $(shell $(CAT) $*.paper.make))); \
	if [ x"$$?" = x"0" ]; then \
	    $(if $(VERBOSE),$(CAT) $@.log,:); \
	    $(MV) '$@.temp' '$@'; \
	else \
	    $(CAT) $@.log; \
	    $(call remove-temporary-files,'$@.temp'); \
	    $(sh_false); \
	fi

# Build the final dvi file.  This is a very tricky rule because of the way that
# latex runs multiple times, needs graphics after the first run (or maybe
# already has them), and relies on bibliographies or indices that may not exist.
#
#	Check the log for fatal errors.  If they exist, colorize and bail.
#
#	Create the .auxdvi.cookie file.  (Needed for next time if not present)
#
#	If any of the following are true, we must rebuild at least one time:
#
#	* the .bbl was recently rebuilt
#
#		check a cookie, then delete it
#
#	* any of several output files was created or changed:
#
#		check $*.run.cookie, then delete it
#
#	* the .aux file changed in a way that necessitates attention
#
#		Note that if the .auxdvi.make file doesn't exist, this means
#		that we are doing a clean build, so it doesn't figure into the
#		test for running again.
#
#		compare against .auxdvi.make
#
#		move if different, remove if not
#
#	* the .log file has errors or warnings requiring at least one more run
#
#	We use a loop over a single item to simplify the process of breaking
#	out when we find one of the conditions to be true.
#
#	If we do NOT need to run latex here, then we move the $@.1st.make file
#	over to $@ because the .dvi file has already been built by the first
#	dependency run and is valid.
#
#	If we do, we delete that cookie file and do the normal multiple-runs
#	routine.
#
.SECONDARY: $(all_dvi_targets)
%.dvi: %.bbl %.aux
	$(QUIET)\
	fatal=`$(call colorize-latex-errors,$*.log)`; \
	if [ x"$$fatal" != x"" ]; then \
		$(ECHO) "$$fatal"; \
		exit 1; \
	fi; \
	$(call make-auxdvi-file,$*.aux.make,$*.auxdvi.cookie); \
	run=0; \
	for i in 1; do \
		if $(call test-exists,$*.bbl.cookie); then \
			run=1; \
			break; \
		fi; \
		if $(call test-exists,$*.run.cookie); then \
			run=1; \
		    	break; \
		fi; \
		if $(call \
		test-exists-and-different,$*.auxdvi.cookie,$*.auxdvi.make);\
		then \
			run=1; \
			break; \
		fi; \
		if $(call test-log-for-need-to-run,$*); then \
			run=1; \
			break; \
		fi; \
	done; \
	$(call remove-temporary-files,$*.bbl.cookie $*.run.cookie); \
	$(MV) $*.auxdvi.cookie $*.auxdvi.make; \
	if [ x"$$run" = x"1" ]; then \
		$(call remove-files,$@.1st.make); \
		for i in 2 3 4 5; do \
			$(if $(findstring 3.79,$(MAKE_VERSION)),\
				$(call echo-build,$*.tex,$@,$$$$i),\
				$(call echo-build,$*.tex,$@,$$i)\
			); \
			$(call run-latex,$*); \
			$(call test-run-again,$*) || break; \
		done; \
	else \
		$(MV) $@.1st.make $@; \
	fi; \
	$(call latex-color-log,$*)

# Build the .bbl file.  When dependencies are included, this will (or will
# not!) depend on something.bib, which we detect, acting accordingly.  The
# dependency creation also produces the %.auxbbl.make file.  BibTeX is a bit
# finicky about what you call the actual files, but we can rest assured that if
# a .auxbbl.make file exists, then the .aux file does, as well.  The
# .auxbbl.make file is a cookie indicating whether the .bbl needs to be
# rewritten.  It only changes if the .aux file changes in ways relevant to .bbl
# creation.
#
# Note that we do NOT touch the .bbl file if there is no need to
# create/recreate it.  We would like to leave existing files alone if they
# don't need to be changed, thus possibly avoiding a rebuild trigger on the
# .dvi side.
%.bbl: %.auxbbl.make
	$(QUIET)\
	$(if $(filter %.bib,$^),\
		$(call echo-build,$(filter %.bib,$?) $*.aux,$@); \
		$(call run-bibtex,$*); \
		$(TOUCH) $@.cookie; \
	)

# Create the index file
%.ind:	%.idx %.tex
	$(QUIET)$(call echo-build,$<,$@)
	$(QUIET)$(call run-makeindex,$*)
#
# SCRIPTED LaTeX TARGETS
#
.SECONDARY: $(all_tex_targets)
%.tex:	%.tex.sh
	$(QUIET)$(call echo-build,$<,$@)
	$(QUIET)$(SHELL) $< $@

%.tex:	%.rst $(rst_style_file)
	$(QUIET)$(call echo-build,$<,$@)
	$(QUIET)$(call convert-rst,$<,$@)

#
# GRAYSCALE LaTeX TARGETS
#

# Parse %.d to get all of the include files, then run sed to generate new files
# for all of them that depend on _gray.
%._gray_.tex: %.d %.tex
	$(QUIET)$(call echo-build,$^,$@)
	$(QUIET)\
	texstems=`$(SED) \
		 -e 's/[^:]*:[[:space:]]*\(.*\)\.tex[[:space:]]*$$/\\1/p' \
		 -e 'd' \
		 $<`; \
	for f in $$texstems; do \
		$(SED) \
		-e 's/\.eps/._gray_&/' \
		-e 's/\.pstex/._gray_&/' \
		-e 's/\.pstex_t/._gray_&/' \
		-e 's/_include_/&._gray_/g' \
		$$f.tex > $$f._gray_.tex; \
	done;

#
# GRAPHICS TARGETS
#
.PHONY: all-graphics
all-graphics:	$(all_graphics_targets);

.PHONY: all-pstex all-gray-pstex
all-pstex:	$(all_pstex_targets);
all-gray-pstex:	$(all_gray_pstex_targets);

.PHONY: show-graphics
show-graphics: all-graphics
	$(VIEW_GRAPHICS) $(all_known_graphics)

$(gray_eps_file):
	$(QUIET)$(call echo-build,$^,$@)
	$(QUIET)$(call create-gray-eps-file,$@)

%._gray_.eps:	%.gpi $(gpi_sed)
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-gpi,$<,$@,1)

%._gray_.eps:	%.fig
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-fig,$<,$@,1)

%._gray_.eps: %.dot $(gray_eps_file)
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-dot,$<,$@,$<.log,1)

%._gray_.eps: %.eps.gz $(gray_eps_file)
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-epsgz,$<,$@,1)

%._gray_.eps: %.eps $(gray_eps_file)
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-eps,$<,$@,1)

%._gray_.pstex: %.fig
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-fig-pstex,$<,$@,1)

%._gray_.pstex_t: %.fig %._gray_.pstex
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-fig-pstex-t,$<,$@,$*._gray_.pstex,1)

%.eps:	%.gpi $(gpi_sed)
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-gpi,$<,$@,$(GRAY))

%.eps: %.fig
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-fig,$<,$@,$(GRAY))

%.eps: %.dot $(if $(GRAY),$(gray_eps_file))
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-dot,$<,$@,$<.log,$(GRAY))

%.eps: %.eps.gz $(if $(GRAY),$(gray_eps_file))
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-epsgz,$<,$@,$(GRAY))

%.pstex: %.fig
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-fig-pstex,$<,$@,$(GRAY))

%.pstex_t: %.fig %.pstex
	$(QUIET)$(call echo-graphic,$^,$@)
	$(QUIET)$(call convert-fig-pstex-t,$<,$@,$*.pstex,$(GRAY))

#
# DEPENDENCY-RELATED TARGETS.
#

# Generate all of the information needed to get dependencies
# As a side effect, this creates a .dvi file.  We need to be sure to remove it
# if there are errors.  Errors can take several forms and all of them are found
# within the log file:
#	* There was a LaTeX error
#	* A needed file was not found
#	* Cross references need adjustment
#
# Behavior:
#	This rule is responsible for generating the following:
#	%.aux
#	%.d
#	%.aux.make
#	%.dvi.1st.make (the .dvi file, moved)
#
#	Steps:
#
#	Run latex
#	Move .dvi somewhere else (make no judgements about success)
#	Flatten the .aux file into another file
#	Add source dependencies
#	Add graphic dependencies
#	Add bib dependencies
#
#	Create cookies for various suffixes that may represent files that
#	need to be read by LaTeX in order for it to function properly.
#
%.d %.aux %.aux.make: %.tex
	$(QUIET)$(call echo-build,$<,$*.d $*.dvi,1)
	$(QUIET)\
	$(call run-latex,$<,--recorder) || $(sh_true); \
	$(call die-on-pstexs,$*.log); \
	$(MV) $*.dvi $*.dvi.1st.make; \
	$(call flatten-aux,$*.aux,$*.aux.make); \
	$(ECHO) "# vim: ft=make" > $*.d; \
	$(ECHO) ".PHONY: $*._graphics" >> $*.d; \
	$(call get-inputs,$*.fls,$(addprefix $*.,aux aux.make d dvi)) >> $*.d; \
	$(call get-graphics,$*.log,$(addprefix $*.,d dvi _graphics)) >> $*.d; \
	$(call get-inds,$*.log,$(addprefix $*.,d aux aux.make)) >> $*.d; \
	$(call get-bibs,$*.aux.make,$(addprefix $*.,bbl aux aux.make)) >> $*.d; \
	for s in toc out lot lof nav; do \
		if [ -e "$*.$$s" ]; then \
			if ! $(DIFF) -q $*.$$s $*.$$s.make 2>/dev/null; then \
				$(TOUCH) $*.run.cookie; \
			fi; \
			$(CP) $*.$$s $*.$$s.make; \
		fi; \
	done

# This is a cookie that is updated if the flattened aux file has changed in a
# way that affects the bibliography generation.
.SECONDARY: $(addsuffix .auxbbl.make,$(stems_ssg))
%.auxbbl.make: %.aux.make
	$(QUIET)\
	$(call make-auxbbl-file,$<,$@.temp); \
	$(call replace-if-different-and-remove,$@.temp,$@)

# Build a dependency file for .gpi files.  These often plot data files that
# also reside in the directory, so if a data file changes, it's nice to know
# about it.  This also handles loaded .gpi files, whose filename should have
# _include_. in it.
%._gray_.gpi.d: %.gpi
	$(QUIET)$(call echo-build,$<,$@)
	$(QUIET)$(call make-gpi-d,$<,$@)

%.gpi.d: %.gpi
	$(QUIET)$(call echo-build,$<,$@)
	$(QUIET)$(call make-gpi-d,$<,$@)

# Store the paper size for this document -- note that if beamer is used we set
# it to the special BEAMER paper size.  We only do this, however, if the
# special comment exists, in which case we enlarge the output with psnup.
#
#	The paper size is extracted from a documentclass attribute.
%.paper.make: %.tex
	$(QUIET)$(SED) \
	-e '/\\documentclass/,/}/{' \
	-e '  s/%.*//' \
	-e '  H' \
	-e '  /}/{' \
	-e '    s/.*//' \
	-e '    x' \
	-e '    /\\documentclass/!d' \
	-e '    s/[\n[:space:]]*//g' \
	-e '    s/\([,{[]\)\([[:alnum:]]\{1,\}\)paper\([],}]\)/\1%-\2-%\3/g' \
	-e '    s/\([,{[]\)\(landscape\)\([],}]\)/\1%-\2-%\3/g' \
	-e '    s/^[^%]*%-//' \
	-e '    s/-%[^%]*$$//' \
	-e '    s/-%[^%]%-/ /g' \
	-e '    p' \
	-e '  }' \
	-e '  d' \
	-e '}' \
	-e 'd' \
	$< > $@; \
	$(EGREP) -q '^[^%]*\\documentclass[^{]*{beamer}' $< && \
	(\
		$(EGREP) -q '^%%[[:space:]]*BEAMER[[:space:]]*LARGE$$' $< && \
		$(ECHO) "BEAMER" > $@ || \
		: > $@ \
	) || $(sh_true)

# Store embedding instructions for this document using a special comment
%.embed.make: %.tex
	$(QUIET)$(EGREP) '^%%[[:space:]]*NO[[:space:]]*EMBED[[:space:]]*$$' $< \
		&& $(ECHO) '' > $@ \
		|| $(ECHO) '1' > $@;

#
# HELPFUL PHONY TARGETS
#

.PHONY: _all_programs
_all_programs:
	$(QUIET)$(ECHO) "== All External Programs Used =="
	$(QUIET)$(call output-all-programs)

.PHONY: _check_programs
_check_programs:
	$(QUIET)$(ECHO) "== Checking Makefile Dependencies =="; $(ECHO)
	$(QUIET) \
	$(ECHO) hi; \
	allprogs=`\
	 ($(call output-all-programs)) | \
	 $(SED) \
	 -e 's/^[[:space:]]*//' \
	 -e '/^#/d' \
	 -e 's/[[:space:]]*#.*//' \
	 -e '/^=/s/[[:space:]]/_/g' \
	 -e '/^[[:space:]]*$$/d' \
	 -e 's/^[^=].*=[[:space:]]*\([^[:space:]]\{1,\}\).*$$/\\1/' \
	 `; \
	spaces='                             '; \
	for p in $${allprogs}; do \
	case $$p in \
		=*) $(ECHO); $(ECHO) "$$p";; \
		*) \
			$(ECHO) -n "$$p:$$spaces" | $(SED) -e 's/^\(.\{0,20\}\).*$$/\1/'; \
			loc=`$(WHICH) $$p`; \
			if [ x"$$?" = x"0" ]; then \
				$(ECHO) "$(C_SUCCESS)Found:$(C_RESET) $$loc"; \
			else \
				$(ECHO) "$(C_FAILURE)Not Found$(C_RESET)"; \
			fi; \
			;; \
	esac; \
	done

.PHONY: _check_gpi_files
_check_gpi_files:
	$(QUIET)$(ECHO) "== Checking all .gpi files for common errors =="; \
	$(ECHO); \
	for f in $(files.gpi); do \
	result=`$(EGREP) '^([^#]*set terminal |set output )' $$f`; \
	$(ECHO) -n "$$f: "; \
	if [ x"$$result" = x"" ]; then \
		$(ECHO) "$(C_SUCCESS)Okay$(C_RESET)"; \
	else \
		$(ECHO) "$(C_FAILURE)Warning: Problematic commands:$(C_RESET)";\
		$(ECHO) "$(C_ERROR)$$result$(C_RESET)"; \
	fi; \
	done; \
	$(ECHO)

.PHONY: _all_stems
_all_stems:
	$(QUIET)$(ECHO) "== All Stems =="
	$(QUIET)$(call echo-list,$(sort $(all_stems)))

.PHONY: _includes
_includes:
	$(QUIET)$(ECHO) "== Include Stems =="
	$(QUIET)$(ECHO) "=== Sources ==="
	$(QUIET)$(call echo-list,$(sort $(source_includes)))
	$(QUIET)$(ECHO) "=== Graphics ==="
	$(QUIET)$(call echo-list,$(sort $(graphic_includes)))

.PHONY: _all_sources
_all_sources:
	$(QUIET)$(ECHO) "== All Sources =="
	$(QUIET)$(call echo-list,$(sort $(all_files.tex)))

.PHONY: _dependency_graph
_dependency_graph:
	$(QUIET)$(ECHO) "/* LaTeX Dependency Graph */"
	$(QUIET)$(call output-dependency-graph)

.PHONY: _show_dependency_graph
_show_dependency_graph:
	$(QUIET)$(call output-dependency-graph,$(graph_stem).dot)
	$(QUIET)$(DOT) -Tps -o $(graph_stem).eps $(graph_stem).dot
	$(QUIET)$(VIEW_POSTSCRIPT) $(graph_stem).eps
	$(QUIET)$(call remove-temporary-files,$(graph_stem).*)

.PHONY: _sources
_sources:
	$(QUIET)$(ECHO) "== Sources =="
	$(QUIET)$(call echo-list,$(sort $(files.tex)))

.PHONY: _scripts
_scripts:
	$(QUIET)$(ECHO) "== Scripts =="
	$(QUIET)$(call echo-list,$(sort $(files_scripts)))

.PHONY: _graphic_outputs
_graphic_outputs:
	$(QUIET)$(ECHO) "== Graphic Outputs =="
	$(QUIET)$(call echo-list,$(sort $(all_graphics_targets)))

.PHONY: _graphic_sources
_graphic_sources:
	$(QUIET)$(ECHO) "== Graphic Sources =="
	$(QUIET)$(call echo-list,$(sort $(files_graphics)))

.PHONY: _env
_env:
ifdef .VARIABLES
	$(QUIET)$(ECHO) "== MAKE VARIABLES =="
	$(QUIET)$(call echo-list,$(foreach var,$(sort $(.VARIABLES)),'$(var)'))
endif
	$(QUIET)$(ECHO) "== ENVIRONMENT =="
	$(QUIET)$(ENV)

#
# CLEAN TARGETS
#
.PHONY: clean-deps
clean-deps:
	$(QUIET)$(call remove-files,$(all_d_targets) *.make *.make.temp *.cookie)

.PHONY: clean-tex
clean-tex: clean-deps
	$(QUIET)$(call remove-files,$(rm_tex))

.PHONY: clean-graphics
# TODO: This *always* deletes pstex files, even if they were not generated by
# anything....  In other words, if you create a pstex and pstex_t pair by hand
# an drop them in here without the generating fig file, they will be deleted
# and you won't get them back.  It's a hack put in here because I'm not sure we
# even want to keep pstex functionality, so my motivation is not terribly high
# for doing it right.
clean-graphics:
	$(QUIET)$(call remove-files,$(all_graphics_targets) *.gpi.d *.pstex *.pstex_t)

.PHONY: clean-backups
clean-backups:
	$(QUIET)$(call remove-files,$(backup_patterns) *.temp)

.PHONY: clean-auxiliary
clean-auxiliary:
	$(QUIET)$(call remove-files,$(graph_stem).*)

.PHONY: clean-nographics
clean-nographics: clean-tex clean-deps clean-backups clean-auxiliary ;

.PHONY: clean
clean:	clean-tex clean-graphics clean-deps clean-backups clean-auxiliary

#
# HELP TARGETS
#

.PHONY: help
help:
	$(help_text)

.PHONY: version
version:
	$(QUIET)\
	$(ECHO) "$(fileinfo) Version $(version)"; \
	$(ECHO) "by $(author)"; \
	$(ECHO); \
	$(ECHO) 'SVN info: $(svninfo)';

#
# HELP TEXT
#

define help_text
# $(fileinfo) Version $(version)
#
# by $(author)
#
# Generates a number of possible output files from a LaTeX document and its
# various dependencies.  Handles .bib files, \include and \input, and .eps
# graphics.  All dependencies are handled automatically by running LaTeX over
# the source.
#
# USAGE:
#
#    make [GRAY=1] [VERBOSE=1] [SHELL_DEBUG=1] <target(s)>
#
# STANDARD OPTIONS:
#    GRAY:
#        Setting this variable forces all recompiled graphics to be grayscale.
#        It is useful when creating a document for printing.  The default is
#        to allow colors.  Note that it only changes graphics that need to be
#        rebuilt!  It is usually a good idea to do a 'make clean' first.
#
#        There is another facility for creating grayscale documents that is
#        better when you can use it (it has some small limitations not shared
#        by this approach).  See the section on %._gray_ targets below.
#
#    VERBOSE:
#        This turns off all @ prefixes for commands invoked by make.  Thus,
#        you get to see all of the gory details of what is going on.
#
#    SHELL_DEBUG:
#        This enables the -x option for sh, meaning that everything it does is
#        echoed to stderr.  This is particularly useful for debugging
#        what is going on in $$(shell ...) invocations.  One of my favorite
#        debugging tricks is to do this:
#
#        make -d SHELL_DEBUG=1 VERBOSE=1 2>&1 | less
#
# STANDARD ENVIRONMENT VARIABLES:
#
#      LATEX_COLOR_WARNING		'$(LATEX_COLOR_WARNING)'
#      LATEX_COLOR_ERROR		'$(LATEX_COLOR_ERROR)'
#      LATEX_COLOR_UNDERFULL		'$(LATEX_COLOR_UNDERFULL)'
#      LATEX_COLOR_OVERFULL		'$(LATEX_COLOR_OVERFULL)'
#      LATEX_COLOR_PAGES		'$(LATEX_COLOR_PAGES)'
#      LATEX_COLOR_BUILD		'$(LATEX_COLOR_BUILD)'
#      LATEX_COLOR_GRAPHIC		'$(LATEX_COLOR_GRAPHIC)'
#      LATEX_COLOR_DEP			'$(LATEX_COLOR_DEP)'
#      LATEX_COLOR_SUCCESS		'$(LATEX_COLOR_SUCCESS)'
#      LATEX_COLOR_FAILURE		'$(LATEX_COLOR_FAILURE)'
#
#   These may be redefined in your environment to be any of the following:
#
#      black
#      red
#      green
#      yellow
#      blue
#      magenta
#      cyan
#      white
#
#   Bold or underline may be used, as well, either alone or in combination
#   with colors:
#
#      bold
#      uline
#
#   Order is not important.  You may want, for example, to specify:
#
#   export LATEX_COLOR_SUCCESS='bold blue uline'
#
#   in your .bashrc file.  I don't know why, but you may want to.
#
# STANDARD TARGETS:
# 
#    all:
#        Make all possible documents in this directory.  The documents are
#        determined by scanning for .tex and .tex.sh (described in more detail
#        later) and omitting any file that ends in ._include_.tex or
#        ._nobuild_.tex.  The output is a set of .pdf files.
#
#        If you wish to omit files without naming them with the special
#        underscore names, set the following near the top of the Makefile,
#        or (this is recommended) within a Makefile.ini in the same directory:
#
#        	includes.tex := file1.tex file2.tex
#
#        This will cause the files listed to be considered as include files.
#
#        If you have only few source files, you can set
#
#        	onlysources.tex := main.tex
#
#        This will cause only the source files listed to be considered in
#        dependency detection.  All other .tex files will be considered as
#        include files.  Note that these options work for *any* source type,
#        so you could do something similar with includes.gpi, for example.
#
#    show:
#        Builds and displays all documents in this directory.  It uses the
#        environment-overridable value of VIEW_PDF (currently $(VIEW_PDF)) to
#        do its work.
#
#    all-graphics:
#        Make all of the graphics in this directory.
#
#    all-pstex:
#        Build all fig files into pstex and pstex_t files.  Gray DOES NOT WORK.
#
#    show-graphics:
#        Builds and displays all graphics in this directory.  Uses the
#        environment-overridable value of VIEW_GRAPHICS (currently
#        $(VIEW_GRAPHICS)) to do its work.
#
#    clean:
#        Remove ALL generated files, leaving only source intact.
#
#    clean-graphics:
#        Remove all generated graphics files.
#
#    clean-backups:
#        Remove all backup files: $(backup_patterns)
#        (XFig and other editors have a nasty habit of leaving them around)
#        Also removes Makefile-generated .temp files
#
#    clean-tex:
#        Remove all files generated from LaTeX invocations except dependency
#        information.  Leaves graphics alone.
#
#    clean-deps:
#        Removes all auto-generated dependency information.
#
#    clean-auxiliary:
#        Removes extra files created by various targets (like the dependency
#        graph output).
#
#    clean-nographics:
#        Cleans everything *except* the graphics files.
#
#    help:
#        This help text.
#
#    version:
#        Version information about this LaTeX makefile.
#
# DEBUG TARGETS:
#
#    _all_programs:
#        A list of the programs used by this makefile.
#
#    _check_programs:
#        Checks your system for the needed software and reports what it finds.
#
#    _check_gpi_files:
#        Checks the .gpi files in the current directory for common errors, such
#        as specification of the terminal or output file inside of the gpi file
#        itself.
#
#    _dependency_graph:
#        Outputs a .dot file to stdout that represents a graph of LaTeX
#        dependencies.  To see it, use the _show_dependency_graph target or
#        direct the output to a file, run dot on it, and view the output, e.g.:
#
#        make _dependency_graph > graph.dot
#        dot -T ps -o graph.eps graph.dot
#        gv graph.eps
#
#    _show_dependency_graph:
#        Makes viewing the graph simple: extracts, builds and displays the
#        dependency graph given in the _dependency_graph target using the value
#        of the environment-overridable VIEW_POSTSCRIPT variable (currently set
#        to $(VIEW_POSTSCRIPT)).  The postscript viewer is used because it
#        makes it easier to zoom in on the graph, a critical ability for
#        something so dense and mysterious.
#
#    _all_sources:
#        List all .tex files in this directory.
#
#    _sources:
#        Print out a list of all compilable sources in this directory.  This is
#        useful for determining what make thinks it will be using as the
#        primary source for 'make all'.
#
#    _scripts:
#        Print out a list of scripts that make knows can be used to generate
#        .tex files (described later).
#
#    _all_stems:
#        Print a list of stems.  These represent bare targets that can be
#        executed.  Listing <stem> as a bare target will produce <stem>.pdf.
#
#    _includes:
#        A list of .d files that would be included in this run if _includes
#        weren't specified.  This target may be used alone or in conjunction
#        with other targets.
#
#    _graphic_sources:
#        A list of all files that can create .eps files
#
#    _graphic_outputs:
#        A list of all generated .eps files
#
#    _env:
#        A list of environment variables and their values.  If supported by
#        your version of make, also a list of variables known to make.
#
# FILE TARGETS:
#
#    %, %.pdf:
#        Build a PDF file from the corresponding %.tex file.  This is
#        done using dvips and ps2pdf.  Some may object to this idea,
#        saying that pdflatex is a better approach, but I disagree for
#        two major reasons:
#
#        * Postscript can be a very nice thing to have directly from the LaTeX
#          file, especially when printing.
#
#        * One word: psfrag.  If you don't know this wonderful package, get to
#          know it.  It is a workhorse for making graphs pretty.
#
#    %._show:
#        A phony target that builds the pdf file and then displays it using the
#        environment-overridable value of VIEW_PDF ($(VIEW_PDF)).
#
#    %._graphics:
#        A phony target that generates all graphics on which %.dvi
#        depends.
#
#    %.ps:
#        Build a Postscript file from the corresponding %.tex file.
#        This is done using dvips.  Paper size is automatically
#        extracted from the declaration
#
#        \documentclass[<something>paper]
#
#        or it is the system default.
#
#        If using beamer (an excellent presentation class), the paper
#        size is ignored.  More on this later.
#
#    %.dvi:
#        Build the DVI file from the corresponding %.tex file.
#
#    %.ind:
#        Build the index for this %.tex file.
#
#    %.eps:
#        Build an eps file from one of the following file types:
#
#       .dot    : graphviz
#       .gpi    : gnuplot
#       .fig    : xfig
#       .eps.gz : gzipped eps
#
#       The behavior of this makefile with each type is described in
#       its own section below.
#
#    %.pstex{,_t}:
#       Build a .pstex_t file from a .fig file.
#
#    All targets have a corresponding %._gray_.suffix form, which creates
#    everything in monochrome.  This is useful for creating both color and
#    grayscale versions of the same document, and they can coexist happily in
#    the same directory.  Examples:
#
#       make test._gray_._graphics 	# Build all grayscale graphics
#       make test._gray_		# Build a grayscale document
#
#    The use of a ._gray_ target creates ._gray_.tex files (not forgetting the
#    included files!) with appropriate dependencies on ._gray_.eps graphics.
#    This approach is in many ways superior to specifying GRAY=1 on the command
#    line, but has some limitations.  Because a new .tex file must be created,
#    this means that the original .tex file must be parsed and all references
#    to graphics and include files must be transformed.  This can be a brittle
#    operation in a macro-based language like LaTeX, since it is very easy to
#    define macros that call \include or \input indirectly.
#
#    Here the naming strategy for include files comes into play.  They all have
#    ._include_. in their name, and are therefore fairly easy to search out.
#    That sequence is unlikely to appear in text, so it is fairly safe to
#    replace it.  Anything ending in .eps is also replaced to end with
#    ._gray_.eps, and is subject to the same issues.
#
#    In short, if your file contains _include_ when not referencing a file, or
#    it says .eps when not referencing a graphic, this approach is probably not
#    for you.  I imagine that these cases are fairly rare, however, so it
#    should work most of the time.  When a doubt arises, you can be sure that
#    GRAY=1 will do the right thing, provided you precede it with a 'make
#    clean'.
#
# FEATURES:
#
#    External Program Dependencies:
#        Every external program used by the makefile is represented by an
#        ALLCAPS variable at the top of this file.  This should allow you to
#        make judgments about whether your system supports the use of this
#        makefile.  The list is available in the ALL_PROGRAMS variable and,
#        provided that you are using GNU make 3.80 or later (or you haven't
#        renamed this file to something weird like "mylatexmakefile" and like
#        invoking it with make -f) can be viewed using
#
#        make _all_programs
#
#        Additionally, the availability of these programs can be checked
#        automatically for you by running
#
#        make _check_programs
#
#        The programs are categorized according to how important they are and
#        what function they perform to help you decide which ones you really
#        need.
#
#    Colorized Output:
#        The output of commands is colorized to highlight things that are often
#        important to developers.  This includes {underfull,overfull}
#        {h,v}boxes, general LaTeX Errors, each stage of document building, and
#        the number of pages in the final document.  The colors are obtained
#        using 'tput', so colorization should work pretty well on any terminal.
#
#        The colors can be customized very simply by setting any of the
#        LATEX_COLOR_<CONTEXT> variables in your environment (see above).
#
#    Predecessors to TeX Files:
#        Given a target <target>, if no <target>.tex file exists but a
#        corresponding script or predecessor file exists, then appropriate
#        action will be taken to generate the tex file.
#
#        Currently supported script or predecessor languages are:
#
#        sh:     %.tex.sh
#
#           Calls the script using sh, assuming that its output is a .tex
#           file.  Of course, your .sh file can call another script to do
#           its work.  Go wild!
#
#           The script is called thus:
#
#              <interpreter> <script file name> <target tex file>
#
#           and therefore sees exactly one parameter: the name of the .tex
#           file that it is to create.
#
#           Why does this feature exist?  I ran into this while working on
#           my paper dissertation.  I wrote a huge bash script that used a
#           lot of sed to bring together existing papers in LaTeX.  It
#           would have been nice had I had something like this to make my
#           life easier, since as it stands I have to run the script and
#           then build the document with make.  This feature provides hooks
#           for complicated stuff that you may want to do, but that I have
#           not considered.
#
#           This approach does not work for included .tex files.  If you
#           want to do something special with those, you should wrap all of
#           that functionality into a top-level source script that creates
#           the necessary includes as well.
#
#        reST:	 %.rst
#
#           Runs the reST to LaTeX converter to generate a .tex file
#           If it finds a file names _rststyle_._include_.tex, uses it as
#           the "stylesheet" option to rst2latex.
#
#    Dependencies:
#
#        In general, dependencies are extracted directly from LaTeX output on
#        your document.  This includes
#
#        *    Bibliography information
#        *    \include or \input files (honoring \includeonly, too)
#        *    Graphics files inserted by the graphicx package
#
#        Where possible, all of these are built correctly and automatically.
#        In the case of graphics files, these are generated from the following
#        file types:
#
#        GraphViz:      .dot
#        GNUPlot:       .gpi
#        XFig:          .fig
#        GZipped EPS:   .eps.gz
#
#        If the file exists as a .eps already, it is merely used (and will not
#        be deleted by 'clean'!).
#
#        LaTeX and BibTeX are invoked correctly and the "Rerun to get
#        cross-references right" warning is heeded a reasonable number of
#        times.  In my experience this is enough for even the most troublesome
#        documents, but it can be easily changed (if LaTeX has to be run after
#        BibTeX more than three times, it is likely that something is moving
#        back and forth between pages, and no amount of LaTeXing will fix
#        that).
#
#        \includeonly is honored by this system, so files that are not
#        specified there will not trigger a rebuild when changed.
#
#    Beamer:
#        A special TeX source comment is recognized by this makefile:
#
#        %%[[:space:]]*BEAMER[[:space:]]*LARGE
#
#        The presence of this comment forces the output of dvips through psnup
#        to enlarge beamer slides to take up an entire letter-sized page.  This
#        is particularly useful when printing transparencies or paper versions
#        of the slides.  For some reason landscape orientation doesn't appear
#        to work, though.
#
#        If you want to put multiple slides on a page, use this option and then
#        print using mpage, a2ps, or psnup to consolidate slides.  My personal
#        favorite is a2ps, but your mileage may vary.
#
#        When beamer is the document class, dvips does NOT receive a paper size
#        command line attribute, since beamer does special things with sizes.
#
#    GNUPlot Graphics:
#        When creating a .gpi file, DO NOT INCLUDE the "set terminal" or "set
#        output" commands!  The makefile will include terminal information for
#        you.  Besides being unnecessary and potentially harmful, including the
#        terminal definition in the .gpi file makes it harder for you, the one
#        writing the document, to preview your graphics, e.g., with
#
#           gnuplot -persist myfile.gpi
#
#        so don't do specify a terminal or an output file in your .gpi files.
#
#        When building a gpi file into an eps file, there are several features
#        available to the document designer:
#
#        Global Header:
#            The makefile searches for the files in the variable GNUPLOT_GLOBAL
#            in order:
#
#            ($(GNUPLOT_GLOBAL))
#
#            Only the first found is used.  All .gpi files in the directory are
#            treated as though the contents of GNUPLOT_GLOBAL were directly
#            included at the top of the file.
#
#            NOTE: This includes special comments! (see below)
#
#        Font Size:
#            A special comment in a .gpi file (or a globally included file) of
#            the form
#
#            ## FONTSIZE=<number>
#
#            will change the font size of the GPI output.  If font size is
#            specified in both the global file and the GPI file, the
#            specification in the individual GPI file is used.
#
#        Grayscale Output:
#            GNUplot files also support a special comment to force them to be
#            output in grayscale *no matter what*:
#
#            ## GRAY
#
#            This is not generally advisable, since you can always create a
#            grayscale document using the forms mentioned above.  But, if your
#            plot simply must be grayscale even in a document that allows
#            colors, this is how you do it.    
#
#    XFig Graphics:
#            No special handling is done with XFig, except when a global
#            grayscale method is used, e.g.
#
#                make document._gray_
#                or
#                make GRAY=1 document
#
#            In these cases the .eps files is created using the -N switch to
#            fig2dev to turn off color output.  (Only works with eps, not
#            pstex output!)
#
#    GraphVis Graphics:
#            Color settings are simply ignored here.  The 'dot' program is used
#            to transform a .dot file into a .eps file.
#
#    GZipped EPS Graphics:
#        
#        A .eps.gz file is sometimes a nice thing to have.  EPS files can get
#        very large, especially when created from bitmaps (don't do this if you
#        don't have to).  This makefile will unzip them (not in place) to
#        create the appropriate EPS file.
#
endef

#
# DEPENDENCY CHART:
#
#digraph "g" {
#    rankdir=TB
#    size="9,9"
#    edge [fontsize=12 weight=10]
#    node [shape=box fontsize=14 style=rounded]
#
#    eps [
#        shape=Mrecord
#        label="{{<gpi> GNUplot|<epsgz> GZip|<dot> Dot|<fig> XFig}|<eps> eps}"
#        ]
#    pstex [label="%.pstex"]
#    pstex_t [label="%.pstex_t"]
#    tex_outputs [shape=point]
#    extra_tex_files [shape=point]
#    gpi_data [label="<data>"]
#    gpi_includes [label="_include_.gpi"]
#    aux [label="%.aux"]
#    fls [label="%.fls"]
#    idx [label="%.idx"]
#    ind [label="%.ind"]
#    log [label="%.log"]
#    tex_sh [label="%.tex.sh"]
#    rst [label="%.rst"]
#    tex [
#        shape=record
#        label="<tex> %.tex|<include> _include_.tex"
#        ]
#    include_aux [label="_include_.aux"]
#    file_bib [label=".bib"]
#    bbl [label="%.bbl"]
#    dvi [label="%.dvi"]
#    ps [label="%.ps"]
#    pdf [label="%.pdf"]
#    fig [label=".fig"]
#    dot [label=".dot"]
#    gpi [label=".gpi"]
#    eps_gz [label=".eps.gz"]
#
#    gpi_files [shape=point]
#
#    rst -> tex:tex [label="reST"]
#    tex_sh -> tex:tex [label="sh"]
#    tex -> tex_outputs [label="latex"]
#    tex_outputs -> dvi
#    tex_outputs -> aux
#    tex_outputs -> log
#    tex_outputs -> fls
#    tex_outputs -> idx
#    tex_outputs -> include_aux
#    aux -> bbl [label="bibtex"]
#    file_bib -> bbl [label="bibtex"]
#    idx -> ind [label="makeindex"]
#    ind -> extra_tex_files
#    bbl -> extra_tex_files
#    eps -> extra_tex_files
#    extra_tex_files -> dvi [label="latex"]
#    gpi_files -> eps:gpi [label="gnuplot"]
#    gpi -> gpi_files
#    gpi_data -> gpi_files
#    gpi_includes -> gpi_files
#    eps_gz -> eps:epsgz [label="gunzip"]
#    fig -> eps:fig [label="fig2dev"]
#    fig -> pstex [label="fig2dev"]
#    fig -> pstex_t [label="fig2dev"]
#    pstex -> pstex_t [label="fig2dev"]
#    dot -> eps:dot [label="dot"]
#    dvi -> ps [label="dvips"]
#    include_aux -> bbl [label="bibtex"]
#    ps -> pdf [label="ps2pdf"]
#
#    edge [ color=blue label="" style=dotted weight=1 fontcolor=blue]
#    fls -> tex:include [label="INPUT: *.tex"]
#    fls -> file_bib [label="INPUT: *.aux"]
#    aux -> file_bib [label="\\bibdata{...}"]
#    include_aux -> file_bib [label="\\bibdata{...}"]
#    log -> gpi [label="Graphic file"]
#    log -> fig [label="Graphic file"]
#    log -> eps_gz [label="Graphic file"]
#    log -> dot [label="Graphic file"]
#    log -> idx [label="No such *.ind"]
#    gpi -> gpi_data [label="plot '...'"]
#    gpi -> gpi_includes [label="load '...'"]
#    tex:tex -> ps [label="paper"]
#    tex:tex -> pdf [label="embedding"]
#}

#
# DEPENDENCY CHART SCRIPT
#
# $(call output_dependency_graph,[<output file>])
define output-dependency-graph
	if [ -f '$(this_file)' ]; then \
	$(SED) \
		-e '/^[[:space:]]*#[[:space:]]*DEPENDENCY CHART:/,/^$$/!d' \
		-e '/DEPENDENCY CHART/d' \
		-e '/^$$/d' \
		-e 's/^[[:space:]]*#//' \
		$(this_file) $(if $1,> '$1',); \
	else \
		$(ECHO) "Cannot determine the name of this makefile."; \
	fi
endef
# vim: noet sts=0 sw=8 ts=8

